Domain Adaptation under Open Set Label Shift

We introduce the problem of domain adaptation under Open Set Label Shift (OSLS) where the label distribution can change arbitrarily and a new class may arrive during deployment, but the class-conditional distributions p(x|y) are domain-invariant. OSLS subsumes domain adaptation under label shift and Positive-Unlabeled (PU) learning. The learner's goals here are two-fold: (a) estimate the target label distribution, including the novel class; and (b) learn a target classifier. First, we establish necessary and sufficient conditions for identifying these quantities. Second, motivated by advances in label shift and PU learning, we propose practical methods for both tasks that leverage black-box predictors. Unlike typical Open Set Domain Adaptation (OSDA) problems, which tend to be ill-posed and amenable only to heuristics, OSLS offers a well-posed problem amenable to more principled machinery. Experiments across numerous semi-synthetic benchmarks on vision, language, and medical datasets demonstrate that our methods consistently outperform OSDA baselines, achieving 10--25% improvements in target domain accuracy. Finally, we analyze the proposed methods, establishing finite-sample convergence to the true label marginal and convergence to optimal classifier for linear models in a Gaussian setup. Code is available at https://github.com/acmi-lab/Open-Set-Label-Shift.

==> Open set label shift (NeurIPS 2022)/sections/00_abstract.tex <==
We introduce the problem of domain adaptation 
under Open Set Label Shift (OSLS) \update{where}
the label distribution can change arbitrarily
and a new class may arrive during deployment,
but the class-conditional distributions $p(x|y)$ 
are domain-invariant.
OSLS subsumes domain adaptation under label shift  %(when $p(y=k+1)=0$)
and Positive-Unlabeled (PU) learning.  %(when $k=1$).
The learner's goals here are two-fold:
(a) estimate the target label distribution,
including the novel class;
% \todosg{ Should we say. that this includes novel class as well just to emphasis it? }
and (b) learn a target classifier. %for the target domain. 
First, we establish necessary and sufficient conditions
for identifying these quantities.
Second, motivated by advances in label shift and PU learning,
we propose practical methods for both tasks
that leverage black-box predictors. 
Unlike typical open set domain adaptation problems,
which tend to be ill-posed and amenable only to heuristics, 
OSLS offers a well-posed problem
amenable to more principled machinery. 
Experiments across numerous semi-synthetic 
benchmarks on vision, language,
and medical datasets 
% \todosg{(i.e., MNIST, CIFAR-10, CIFAR-100,
% Newsgroups-20, DermNet, Tabula-Munis and BreakHis)}
demonstrate that our methods
consistently outperform open set domain adaptation  baselines, 
achieving $10$--$25\%$ improvements 
in target domain accuracy. 
Finally, we analyze the proposed methods, 
establishing finite-sample convergence 
to the true label marginal and convergence to
optimal classifier for linear models in a Gaussian setup\footnote{Code is available at \url{https://github.com/acmi-lab/Open-Set-Label-Shift}.}.
% Code is available at \url{https://github.com/Neurips2022Anon}. 


% 
% v2
% 


% Whenever we might anticipate that novel classes could arrive at deployment time,
% we should also expect changes in the relative proportion of previously seen classes. 
% \todosg{I like this line, however, can we emphasis this in intro because this is just one motivation of OSLS. Silly point and nit pick: another motivation can be the reverse which is whenever we observe label shift, we may observe  a new class. ... so I am sure why we choose only this to motivate the OSLS.} 
% To tackle this problem, 
% we introduce domain adaptation 
% under Open Set Label Shift (OSLS), 
% % \todosg{I noticed you completely removed the discussion on OSDA. }
% where $p(y)$ can change arbitrarily, % among previously seen classes,
% a new class $y=k+1$ may arrive at the target time,
% and the class conditional distributions $p(x|y)$ are domain-invariant. 
% Notably, OSLS subsumes label shift (i.e., when $p(y=k+1)=0$)
% and Positive-Unlabeled (PU) learning (i.e., when $k=1$).
% As with these canonical problems, our tasks are two-fold:
% (a) estimate the target label marginal; \todosg{ Should we say. that this includes novel class as well just to emphasis it? }
% and (b) learn a classifier for the target domain. 
% First, we tackle identification,
% establishing necessary and sufficient 
% conditions for producing consistent estimators.
% Second, motivated by the recent label shift and PU learning methods, 
% we propose practical two-stage methods for both tasks. 
% Unlike typical Open Set Domain Adaptation (OSDA) problems,
% % when 
% which
% tend to be ill-posed and amenable only to heuristics, 
% OSLS offers a well-posed open set problem
% amenable to more principled machinery. 
% Experiments across numerous semi-synthetic 
% benchmarks on vision, language,
% and medical datasets 
% \todosg{(i.e., MNIST, CIFAR-10, CIFAR-100,
% Newsgroups-20, DermNet, Tabula-Munis and BreakHis)}
% demonstrate that our methods
% consistently outperform OSDA baselines, 
% achieving $10$--$25\%$ improvements 
% in target domain accuracy. 
% Finally, for the proposed framework, 
% we provide finite-sample convergence 
% results to the true label marginal and 
% show convergence to the true classifier 
% for linear models in a Gaussian setup.
% Code is available at \url{https://github.com/Neurips2022Anon}. 
% % \todosg{Highlight that we are open sourcing the code
% % to replicate and perhaps run more experiments.}
% % \footnote{Code 
% % for our experiments: \url{https://github.com/Neurips2022Anon}}.




% 
% v1
% 

% In Open Set Domain Adaptation (OSDA), 
% we are faced with labeled source data,
% unlabeled target data, and new classes
% may show up in the target data.
% While many heuristics have been proposed for this setting,
% the problem is fundamentally ill-posed absent further assumptions.
% %% 
% To elucidate the basic structure of OSDA,
% we propose \emph{Open Set Label Shift} (OSLS), 
% a well-posed instantiation in which 
% (i) the label distribution 
% $p(y)$ might change among previously seen classes;
% (ii) one new label $y=k+1$ may arrive at target time;
% and (iii) the class conditional distributions $p(x|y)$ 
% remains fixed across domains. 
% Notably, OSLS subsumes label shift 
% and Positive-Unlabeled (PU) learning.
% As with these canonical problems, our tasks are two-fold:
% (i) estimating the target label marginal;
% and (ii) learning a classifier for the target domain. 
% In our work, we first tackle identification,
% establishing some necessary and sufficient 
% conditions for producing consistent estimators.
% %%
% Second, motivated by recent methods
% for label shift and PU learning, 
% we propose practical two-stage methods for both the tasks.  
% % where 
% % our primary contribution is to 
% % lay down the design choices 
% % crucial for performance in 
% % high-dimensional deep learning settings. 
% %% 
% Experiments across numerous semi-synthetic 
% benchmarks on vision and language datasets 
% (i.e., CIFAR-10, Imagenet, SNLI )
% demonstrate that in our setting, 
% the proposed approaches consistently outperform 
% baselines from the OSDA literature, 
% achieving $10$--$25\%$ improvements
% in accuracy on target. 
% %% 
% Finally, for the proposed framework, 
% we provide finite-sample convergence 
% results to the true label marginal and 
% show convergence to the true classifier 
% % in the population 
% for linear models in a Gaussian setup. 



% 
% VERSION 0
% 

% Under Open Set Domain Adaptation (OSDA), 
% our goal is to adapt models trained on 
% % training data (source) to 
% source data to
% % test data (target)
% target data 
% where previously unseen 
% classes may be observed. 
% %%
% Existing work on OSDA largely 
% focus on a general scenario where
% % where along with observing 
% % novel classes
% % in the target domain, the condition 
% distribution among
% previously seen classes changes
% in unspecified way from source to target. 
% However, without precise 
% assumptions on the 
% nature of shift,
% % for previously seen classes 
% the problem of OSDA
% is fundamentally ill-posed. 
% %% 
% In this work, 
% to bring about a systematic 
% progress in the field, 
% we propose 
% \emph{Open Set Label Shift} (OSLS), 
% a principled setting 
% unifying label shift 
% and Positive-Unlabeled (PU) learning where (i) 
% we may observe previously unseen classes; and
% (ii) the label distribution 
% $p(y)$ might change among 
% previously seen classes but the class
% conditional distributions $p(x|y)$ do not. 
% For OSLS, our goal breaks down 
% into two tasks: (i) determining the fraction of 
% all the previously seen classes; and (ii) 
% learning a classifier for the target domain. 
% %%
% In our work, we first 
% establish necessary and sufficient 
% identifiability conditions for this problem. 
% %%
% Second, motivated by recent methods
% for label shift and PU learning, 
% we propose practical 
% two-stage methods for both the tasks.  
% % where 
% % our primary contribution is to 
% % lay down the design choices 
% % crucial for performance in 
% % high-dimensional deep learning settings. 
% %% 
% Experiments across numerous semi-synthetic 
% benchmarks on vision and language datasets 
% (i.e., CIFAR-10, Imagenet, SNLI ) demonstrate 
% that proposed approaches consistently outperform
% alternative baselines from the open set 
% domain adaptation literature, 
% achieving $10$--$25\%$ improvements %placeholder
% in accuracy on target. 
% % we perform large-scale experiments ... 
% %% 
% Finally, for the proposed framework, 
% we provide finite-sample convergence 
% results to the true label marginal and 
% show convergence to the 
% true classifier in population
% for linear models 
% in a Gaussian setup. 

==> Open set label shift (NeurIPS 2022)/sections/01_intro.tex <==
% 
% vn 1
% 
Suppose that we wished to deploy a machine learning system
to recognize diagnoses based on their clinical manifestations.
If the distribution of data were static over time,
then we could rely on the standard machinery of statistical prediction.
However, disease prevalences are constantly changing,
violating the assumption  of independent and identically distributed (iid) data. 
In such scenarios, we might reasonably 
apply the \emph{label shift} assumption,
where prevalences can change but
clinical manifestations cannot.
When only the relative proportion 
of previously seen diseases can change, 
principled methods can detect
and correcting for label shift on the fly
\citep{saerens2002adjusting, zhang2013domain, lipton2018detecting, azizzadenesheli2019regularized, alexandari2019adapting, garg2020labelshift}.
But what if a new disease, like COVID-19,
were to arrive suddenly?

Traditional label shift adaptation techniques break
when faced with a previously unseen class.
A distinct literature on Open Set Domain Adaptation (OSDA) seeks to handle such cases
\citep{panareda2017open, baktashmotlagh2018learning, cao2019learning, tan2019weakly, lian2019known, you2019universal, saito2018open, saito2020universal, fu2020learning}). 
Given access to labeled \emph{source} data and unlabeled \emph{target} data,
the goal in OSDA is to adapt classifiers
in general settings where previous classes
can shift in prevalence (and even appearance),
and novel classes separated 
out from those previously seen can appear.
Most work on OSDA is driven by the creation of 
and progress on benchmark datasets
(e.g., DomainNet, OfficeHome).
Existing OSDA methods are heuristic in nature,
addressing settings where the right answers 
seem intuitive but are not identified mathematically. 
However, absent assumptions on: 
(i) the nature of distribution shift 
among source classes and 
(ii) the relation between source 
classes and novel class, 
standard impossibility results for domain adaptation
condemn us to guesswork~\citep{ben2010impossibility}.
 
\begin{figure*}[t!]
    \centering 
    \subfigure{\includegraphics[width=\linewidth]{figures/OSLS_fig_full.pdf}}
    % \subfigure{\includegraphics[width=0.3\linewidth]{example-image-b}}
    % \vspace{-10pt}
    \caption{\textbf{Left:} \emph{Domain Adaptation under OSLS}. An instantiation of OSDA that applies label shift assumption but allows for a new class to show up in target domain. \textbf{Right:} \emph{Aggregated results across seven semi-synthetic benchmark datasets}. For both target classification and novel class prevalence estimation, PULSE significantly outperforms other methods (lower error is better). For brevity, we only include result for the best OSDA method. For detailed comparison, refer \secref{sec:exp}.   
    }
    % \vspace{-10pt}
    \label{fig:intro}
  \end{figure*}
 

In this work, we introduce domain adaptation
under Open Set Label Shift (OSLS), 
a coherent instantiation of OSDA 
that applies the label shift assumption
but allows for a new class to show up 
in the target distribution.
Formally, the label distribution may shift
between source and target $p_s(y) \neq p_t(y)$,
but the class-conditional distributions 
among previously seen classes may not
(i.e., $\forall y \in \{1,2, \dots,k\}, p_s(x|y) =p_t(x|y)$).
Moreover, a new class $y=k+1$ may arrive 
in the target period. 
Notably, OSLS subsumes label shift~\citep{saerens2002adjusting, storkey2009training, lipton2018detecting} (when $p_t(y=k+1)=0$)
and learning from Positive and Unlabeled (PU) data~\citep{de1999positive, letouzey2000learning, elkan2008learning} (when $k=1$). 
As with label shift and PU learning, 
our goals are two-fold.
Here, we must (i) estimate the target 
label distribution $p_t(y)$ (including the novel class \update{prevalence}); 
(ii) train a $(k+1)$-way target-domain classifier.

First, %we tackle the identification problem
we characterize when the parameters of interest are identified
% introducing both necessary and sufficient conditions
 (\secref{sec:identifiability}). 
Namely, we define a (necessary) \emph{weak positivity} condition,
which states that there exists a subset of each label's support
that has zero probability mass under the novel class
and that \update{the submatrix} of $p(x|y)$ consisting 
only of rows outside the novel class's support is full rank. 
Moreover, we prove that weak positivity alone is not sufficient. 
% Next, 
We introduce two sufficient conditions:
\emph{strong positivity} and \emph{separability},
either of which (independently) ensures identifiability. 
% 
% 

Focusing on cases with {strong positivity},
we show that OSLS reduces 
to $k$ PU learning problems (\secref{sec:reduction}). 
However, we demonstrate that straightforward applications of this idea 
fail because
(i) bias accumulates across the $k$ mixture proportion estimates
leading to grossly underestimating the novel class's prevalence;
and (ii) naive combinations of the $k$ PU classifiers are biased and inaccurate. %OSLS classifiers. 


Thus motivated, we propose the PULSE framework,
which combines methods from Positive and Unlabeled learning
and Label Shift Estimation, 
yielding two-stage techniques for both
label marginal estimation and classification (\secref{sec:framework}). 
Our methods build on recent advances in label shift
\citep{lipton2018detecting, azizzadenesheli2019regularized, alexandari2019adapting, garg2020labelshift} and PU learning \citep{kiryo2017positive,ivanov2019dedpul,garg2021PUlearning}, 
that leverage appropriately chosen black-box predictors  
to avoid the curse of dimensionality.
% 
PULSE first estimates the label shift 
among previously seen classes,
and then re-samples the source data 
to formulate a single PU learning problem 
between (reweighted) source and target data
to estimate fraction of novel class and to learn the target classifier. 
% 
In particular, our procedure builds on the BBE and CVIR 
techniques proposed in \citet{garg2021PUlearning}.
% Z: possibly hint the meta-algorithm is more general (can apply with different choices)
PULSE is simple to implement and compatible 
with arbitrary hypothesis classes (including deep networks). 


We conduct extensive semi-synthetic experiments 
adapting seven benchmark datasets 
spanning vision (CIFAR10, CIFAR100, Entity30), 
natural language (Newsgroups-20), 
biology (Tabula Muris),
and medicine (DermNet, BreakHis)
(\secref{sec:exp}).
Across numerous data modalities, 
draws of the label distributions,
and model architectures,
PULSE consistently outperforms generic OSDA methods, 
improving by $10$--$25\%$ in accuracy on target domain. 
%\todosg{Add one line about failure of OSDA.}
%  
Moreover, PULSE outperforms methods 
that naively solve $k$ PU problems on both 
label distribution estimation and classification.
% 
% Additionally, we observe that without 
% access to any validation labeled data 
% from the target domain, 
% popular OSDA methods significantly 
% under perform as compared to PULSE.


% Next, we ask a natural question: 
% \emph{How do popular methods proposed for 
% OSDA perform in simpler OSLS setting and 
% how do they compare with PULSE?}
% We show that without access to any validation 
% labeled data from the target domain, 
% popular OSDA methods significantly 
% under perform as compared to PULSE (\secref{sec:exp}). 
% We argue that a primary reason 
% underlying the poor performance 
% of OSDA methods are the heuristics 
% employed to detect novel classes. 
% A standard heuristic employed in 
% popular OSDA methods involves 
% thresholding uncertainty 
% estimates at a predefined 
% threshold $\kappa$. However, 
% a fixed $\kappa$, typically doesn't
% work for different datasets and 
% different fractions of 
% the novel class. 
% In contrast, our two-stage method 
% PULSE, first estimates 
% the fraction of novel class which 
% then guides the classification 
% of novel class versus previously seen classes. 

% We evaluate our PULSE framework
% with numerous architectures on 
% six benchmark datasets---adapted to OSLS 
% setting---in vision (e.g, MNIST, CIFAR10, CIFAR100, Imagenet200 ?), 
% NLP (e.g, Newsgroups-20), 
% biology (e.g, Tabula Muris) 
% and medicine (e.g., DermNet, BreakHis)
% which span different modalities, e.g., language, images, tables. 
% Experiments highlight the superiority of PULSE 
% over OSDA 
% baselines across varying novel class fraction 
% and label shift among previously  
% seen classes (\secref{sec:exp}).
% Specifically, PULSE consistently outperform 
% alternative methods, improving by 
% $10$--$25\%$ in accuracy on target domain. 
% Moreover, unlike previous OSDA methods, 
% we highlight the efficacy of PULSE 
% for estimating target label marginal  
% (including the novel class fraction). 
% and label shift among previous seen classes. 

% Since the OSLS framework
% is motivated by applications in 
% medicine and biology, we
% also evaluate the proposed 
% framework on medical 
% and biology datasets.
% We open source the code
% and hope that our experiments on 
% medical datasets encourage other researchers :p 
% 
% Code to replicate our experiments can be found here: \url{https://github.com/Neurips2022Anon}. 


Finally, we analyze our framework (\secref{sec:analysis}).
First, we extend \citet{garg2021PUlearning}'s analysis of BBE
to derive finite-sample error bounds 
for our estimates of the label marginal.
% 
Next, we develop new analyses of the CVIR objective \citep{garg2021PUlearning}
that PULSE relies in the classification stage. 
Focusing on a Gaussian setup and linear models
optimized by gradient descent,
we prove that CVIR converges
to a true positive versus negative classifier in population. 
%
Addressing the overparameterized setting 
where parameters exceed dataset size,
we conduct an empirical study
that helps to elucidate why, on separable data,
CVIR outperforms other consistent objectives,
including nnPU~\citep{kiryo2017positive} and uPU~\citep{du2015convex}.





% 
% vn 0.5
% 

% Suppose that we wished to deploy a machine learning system
% to recognize diagnoses based on their clinical manifestations.
% If the distribution of data were static over time,
% then we could rely on the standard machinery of statistical prediction.
% However, disease prevalences are constantly changing,
% violating the assumption  of independent and identically distributed (iid) data. 
% In such scenarios, we might reasonably 
% apply the \emph{label shift} assumption,
% where prevalences can change but
% clinical manifestations cannot.
% When only the relative proportion 
% of previously seen diseases can change, 
% principled methods can detect
% and correcting for label shift on the fly
% \citep{saerens2002adjusting, zhang2013domain, lipton2018detecting, azizzadenesheli2019regularized, alexandari2019adapting, garg2020unified}.
% But what if a new disease, like COVID-19,
% were to arrive suddenly?


% Traditional label shift adaptation techniques break
% when faced with a previously unseen class.
% A distinct literature on Open Set Domain Adaptation (OSDA) seeks to handle such cases
% \citep{panareda2017open, baktashmotlagh2018learning, cao2019learning, tan2019weakly, lian2019known, you2019universal, saito2018open, saito2020universal, fu2020learning}). 
% Given access to labeled source data and unlabeled target data,
% the goal in OSDA is to adapt classifiers
% in general settings where previous classes
% can shift in prevalence (and even appearance),
% and novel classes must be separated 
% out from those previously seen.
% Most work on OSDA is driven by the creation of 
% and progress on benchmark datasets
% (e.g., DomainNet, OfficeHome).
% Existing OSDA methods are heuristic in nature,
% addressing settings where the right answers 
% seem intuitive but are not identified mathematically. 
% However, absent assumptions on: 
% (i) the nature of distribution shift 
% among source classes and 
% (ii) the relation between source 
% classes and novel class, 
% standard impossibility results for domain adaptation
% condemn us to guesswork~\citep{ben2010impossibility}.
 
% In this work, we introduce Open Set Label Shift (OSLS), 
% a coherent framework for OSDA, 
% where the label shift assumption applies 
% and new classes may arrive at test time.
% Formally, the label distribution may shift
% between source and target $p_s(y) \neq p_t(y)$,
% but the class-conditional distributions 
% among previously seen classes may not
% $\forall y \in \{1,2, \dots,k\}, p_s(x|y) =p_t(x|y)$.
% Moreover, a new class $y=k+1$ may arrive 
% in the target period. 
% Notably, OSLS subsumes label shift~\citep{saerens2002adjusting, storkey2009training, lipton2018detecting} (when $p_t(y=k+1)=0$)
% and learning from Positive and Unlabeled (PU) data~\citep{de1999positive, letouzey2000learning, elkan2008learning} (when $k=1$). 
% As with label shift and PU learning, 
% our goals are two-fold.
% Here, we must (i) estimate the target 
% label distribution $p_t(y)$ (including the novel class); 
% (ii) train a $(k+1)$-way target-domain classifier.




%
%
% v1
%
%

% Machine learning models
% are typically developed and 
% evaluated assuming independent
% and identically distributed (iid)
% data~\citep{ben2010theory}. The rooted underlying 
% assumption is the closed-set 
% classification setting where the training 
% data (source) and test data (target)
% are observed from the same set of predefined 
% classes~\citep{bendale2015towards, panareda2017open}. 
% % 
% However, when deployed in the wild,
% classifiers can be presented 
% with distribution shift problems 
% where we may not only observe a 
% distribution shift from 
% source to target among 
% previously seen classes but 
% samples from \emph{novel}, i.e., 
% classes unseen in source
% can routinely emerge in target~\citep{}. 
% % 
% While it can be hard to distinguish
% between different novel classes 
% with only access to unlabeled target data,
% we can nonetheless hope to 
% separate out novel classes from previously seen. 
% %



% This problem has been studied in the literature 
% as Open Set Domain Adaptation (OSDA;~\citep{panareda2017open, baktashmotlagh2018learning, cao2019learning, tan2019weakly, lian2019known, you2019universal, saito2018open, saito2020universal, fu2020learning}). 
% In particular, given access to 
% labeled source data and 
% unlabeled target data, 
% the goal in OSDA is to 
% learn a classifier that
% can: (i) adapt to the target distribution
% of previously seen classes; and 
% (ii) separate out novel classes 
% in the target. Existing work in OSDA~\citep{saito2020universal, saito2018open, you2019universal, panareda2017open, lian2019known} 
% primarily focuses on scenarios motivated 
% by benchmark datasets (e.g., DomainNet, OfficeHome) where
% the distribution shift from source to target 
% among previously seen classes only satisfy some 
% implicit notion of ``semantic equivalence'' 
% without an explicit characterization 
% of the nature of shift. 
% For example, consider a scenario
% where the source data contain 
% real world images of objects 
% and the target domain comprises of 
% clipart images of source classes 
% and novel classes, 
% as in the popular benchmark of Office-Home 
% dataset~\citep{venkateswara2017deep}.
% However, theory dictates that 
% without assumption  
% on: (i) the nature of distribution shift 
% among source classes and 
% (ii) the relation between source 
% classes and novel class, 
% learning under OSDA is impossible~\citep{ben2010impossibility}.  


% In this work, we introduce
% Open Set Label Shift (OSLS), 
% a principled setting for OSDA 
% that %gracefully
% generalizes label shift~\citep{saerens2002adjusting, storkey2009training, lipton2018detecting} 
% and learning from 
% Positive and Unlabeled (PU) data~\citep{de1999positive, letouzey2000learning, elkan2008learning}. 
% Similar to OSDA, under OSLS, 
% we are given labeled source data 
% and unlabeled target data.
% This setting is characterized by two 
% assumptions: (i) 
% label shift among source classes, i.e., 
% the label distribution $p(y)$
% might change among previously seen 
% classes from source to target 
% but the class-conditional 
% distribution $p(x|y)$
% remain invariant; and 
% (ii) a novel class 
% might be observed
% in unlabeled target data. 
% % 
% % 
% % Note that as special cases, when no novel class 
% % is observed in target(i.e., $p_t(y = k+1) = 0$),
% % we obtain the label shift problem, and 
% % when we observe only one class in source (i.e., $k=1$), 
% % the OSLS problem reduces to PU learning. 
% \todosg{For a reader who is unaware of these two problems can find is annoying here? I removed it -- Maybe I will just have this in setup?} 
% %
% As with label shift and PU learning, 
% the OSLS problem breaks into 
% two sub-tasks: (i) determining the proportion 
% of all the previously seen classes 
% in the target domain, and thereby, 
% estimating the fraction of novel class; and 
% (ii) given such an estimate, train a classifier
% on target domain
% that can adapt to label shift 
% among source classes and 
% identify novel classes. 
% % 


% %% Mot sure what all we should keep, but 
% % I want to motivate the setting very clearly to get people interested in this. 

% Despite its simplicity, the OSLS setting
% is of significant practical relevance. For example,  
% biologists often have labeled database with 
% known cell types (source) 
% and unlabeled database of tissue cells (target)
% which may contain novel cell types~\citep{cao2019learning, elkan2008learning}. 
% They can use the 
% data to train a classifier model and then deploy the
% model to not only identify cell type in a target tissue 
% but also to discover previously unknown cell types. 
% % 
% The OSLS problem can also routinely appear in medical 
% diagnosis where disease cause symptom~\citep{lipton2018detecting}. 
% Along with changing prevalence of known 
% diseases, novel diseases can appear over time. 
% % 
% Additionally, in the presence of 
% significant amount of novel data, 
% estimating the fraction of novel class can
% also trigger appropriate audit response. 
% % 
% Although OSLS setting is relevant and simple,  
% it is largely unexplored. 
% To the best of our knowledge, 
% our paper is the first work 
% exploring OSLS problem 
% in deep learning.


% % In this paper, 
% %% This paragraph needs heavy editing and trimmer, 
% %% Currently I have dumped everything
% To begin making the OSLS problem tractable, 
% we first present identifiability conditions (\secref{sec:identifiability}). 
% % Inspired by label shift, 
% We propose \emph{weak positivity} condition
% which states that there exists
% a subdomain $X_{\wpos} \subseteq \calX $  
% such that no input in $X_\wpos$ belongs 
% to a novel class (i.e., $p( X_\wpos | y = k+1) = 0$)
% and the matrix formed by $p(x|y)$ on 
% inputs in $X_\wpos$ and labels in 
% source classes is full-rank. 
% We show that while weak positivity 
% is necessary for identifiability, 
% it is not sufficient. Next, 
% we extend weak positivity to two stronger conditions: 
% \emph{strong positivity} and \emph{separability}, 
% each of which independently 
% ensure identifiability. \todosg{Removed the extra description from below, we can add if need be!}
% % Intuitively, strong positivity extends weak 
% % positivity by making an additional assumption 
% % that the matrix formed by 
% % $p(x|y)$ on inputs in $X_\wpos$ diagonal. 
% % Seprability assumption extends weak positivity 
% % condition to the full input domain of source classes
% % instead of just $X_\wpos$. 
% % 


% % we propose two-stage method 
% Second, we propose Positive and Unlabeled 
% learning post Label Shift 
% Estimation (PULSE) framework, a two-stage 
% technique for both, 
% label marginal estimation and classification on 
% target domain (\secref{sec:framework}). We build on recent methods in label shift 
% \citep{lipton2018detecting, azizzadenesheli2019regularized, alexandari2019adapting, garg2020labelshift} and 
% PU learning~\citep{kiryo2017positive,ivanov2019dedpul,garg2021PUlearning}, 
% that leverage blackbox classifiers 
% to avoid curse of dimensionality. 
% In particular, our procedure builds on top of BBE and CVIR 
% techniques proposed in \citet{garg2021PUlearning}.
% PULSE is simple to implement and 
% compatible with arbitrary hypothesis classes (including deep networks). 

% The primary methodological contribution 
% of our work in PULSE is to lay down different 
% design choices and outline steps crucial 
% for performance in 
% high-dimensional deep learning settings. 
% % 
% We begin with the observation  
% that we can divide OSLS problem into $k$ PU learning 
% problems. In particular, by treating 
% each source class as positive 
% and unlabeled target data as is, 
% we obtain a positive and unlabeled 
% learning problem. 
% However, we show that naively 
% employing PU learning 
% techniques by training $k$-classifiers 
% for both the tasks  
% scales poorly with increasing $k$.  
% % and produce classifiers that 
% % 
% Instead, by leveraging 
% a source classifier
% we first estimate the label shift among
% previously seen classes, and then 
% employ importance re-weighting of source 
% data to formulate a single PU learning problem 
% between source and target to estimate fraction 
% of novel class and to learn target classifier. 


% Next, we ask a natural question: 
% \emph{How do popular methods proposed for 
% OSDA perform in simpler OSLS setting and 
% how do they compare with PULSE?}
% We show that without access to any validation 
% labeled data from the target domain, 
% popular OSDA methods significantly 
% under perform as compared to PULSE (\secref{sec:exp}). 
% We argue that a primary reason 
% underlying the poor performance 
% of OSDA methods are the heuristics 
% employed to detect novel classes. 
% A standard heuristic employed in 
% popular OSDA methods involves 
% thresholding uncertainty 
% estimates at a predefined 
% threshold $\kappa$. However, 
% a fixed $\kappa$, typically doesn't
% work for different datasets and 
% different fractions of 
% the novel class. 
% In contrast, our two-stage method 
% PULSE, first estimates 
% the fraction of novel class which 
% then guides the classification 
% of novel class versus previously seen classes. 

% We evaluate our PULSE framework
% with numerous architectures on 
% six benchmark datasets---adapted to OSLS 
% setting---in vision (e.g, MNIST, CIFAR10, CIFAR100, Imagenet200 ?), 
% NLP (e.g, Newsgroups-20), 
% biology (e.g, Tabula Muris) 
% and medicine (e.g., DermNet, BreakHis)
% which span different modalities, e.g., language, images, tables. 
% Experiments highlight the superiority of PULSE 
% over OSDA 
% baselines across varying novel class fraction 
% and label shift among previously  
% seen classes (\secref{sec:exp}).
% Specifically, PULSE consistently outperform 
% alternative methods, improving by 
% $10$--$25\%$ in accuracy on target domain. 
% Moreover, unlike previous OSDA methods, 
% we highlight the efficacy of PULSE 
% for estimating target label marginal  
% (including the novel class fraction). 
% % and label shift among previous seen classes. 

% % Since the OSLS framework
% % is motivated by applications in 
% % medicine and biology, we
% % also evaluate the proposed 
% % framework on medical 
% % and biology datasets.
% % We open source the code
% % and hope that our experiments on 
% % medical datasets encourage other researchers :p 
% % 
% % Code to replicate our experiments can be found here: \url{https://github.com/Neurips2022Anon}. 


% Finally, we analyse the proposed 
% framework for OSLS (\secref{sec:analysis}). 
% We present finite-sample error
% analysis for target label marginal
% estimation by simply
% extending the BBE result 
% from \citet{garg2021PUlearning}. 
% % 
% For classification algorithm
% (i.e., CVIR~\citep{garg2021PUlearning})
% employed for PU learning 
% in the second stage of PULSE,  
% we theoretically show that 
% in a Gaussian setup
% with linear models, the alternating 
% procedure with gradient descent will 
% converge to the true positive 
% versus negative classifier in population. 
% % 
% For overparameterized situation, we 
% empirically investigate % change this. 
% CVIR in the controlled Gaussian setup
% and highlight that the main reason 
% behind its efficacy is the 
% early learning phenomena 
% followed by the self-training procedure
% which further improves the 
% accuracy of an otherwise 
% early stopped model. 

% % the 
% % which is ). 
% % While the algorithm was originally
% % proposed in \citet{garg2021PUlearning}, 
% % no analysis was provided for the 
% % alternating CVIR procedure. 

==> Open set label shift (NeurIPS 2022)/sections/02_related.tex <==
\textbf{(Closed Set) Domain Adaptation (DA) {} {}}
Under DA, the goal is to adapt a predictor
from a source distribution with labeled data
% a classifier 
% trained on source data
to a target distribution from which 
we observe only unlabeled examples. 
DA is classically explored under 
two distribution shift scenarios~\citep{storkey2009training}: 
(i) Covariate shift~\citep{zhang2013domain,zadrozny2004learning,cortes2010learning,cortes2014domain,gretton2009covariate}
where $p(y|x)$ remains invariant
among source and target; 
and (ii) Label shift~\citep{saerens2002adjusting, lipton2018detecting, azizzadenesheli2019regularized, alexandari2019adapting, garg2020labelshift, zhang2020coping} where $p(x|y)$
is shared across source and target.
% 
% \citet{scholkopf2012causal} illustrated
% how covariate shift and label shift
% correspond to causal and anti-causal prediction,
% respectively.
% 
% As in these settings,
In these settings most theoretical analysis 
% requires that the source distribution 
requires that the target distribution's support 
is a subset of the source support~\citep{ben2010impossibility}. 
% 
% Notably, \citet{ben2010theory} 
% leverages hypothesis 
% capacity constraints
% to enable generalization to 
% out-of-support samples. 
% 
However, recent empirically work in 
DA~\citep{long2015learning,long2017deep, sun2016deep, sun2017correlation, zhang2019bridging, zhang2018collaborative, ganin2016domain, sohn2020fixmatch}     
focuses on settings 
motivated by benchmark datasets
(e.g., WILDS~\citep{ sagawa2021extending, wilds2021}, 
Office-31~\citep{saenko2010adapting}
OfficeHome~\citep{venkateswara2017deep}, 
DomainNet~\citep{peng2019moment}) 
where such overlap assumptions are violated. 
Instead, they rely on some intuitive
notion of semantic equivalence across domains. 
These problems are not well-specified
and in practice, %despite access to unlabeled data 
despite careful hyperparameter tuning, 
these methods %popular empirical methods  
often do not improve over 
standard empirical risk minimization
on source data alone for practical, 
and importantly, previously unseen
datasets~\citep{sagawa2021extending}.  




 
\textbf{Open Set Domain Adaptation (OSDA) {} {}} 
OSDA~\citep{panareda2017open, bendale2015towards, 6365193}
extends DA to settings where along with distribution 
shift among previously seen classes, 
we may observe a novel class in the target data. 
This setting is also known 
as \emph{universal domain adaptation}~\citep{you2019universal, saito2020universal}. 
\update{Rather than making precise assumptions 
about the nature of shift between source and target as in OSLS}, 
the OSDA literature is primarily governed by 
semi-synthetic problems on benchmark DA datasets
(e.g. DomainNet, Office-31 and OfficeHome). 
Numerous OSDA methods have been proposed~\citep{baktashmotlagh2018learning, cao2019learning, tan2019weakly, lian2019known, you2019universal, saito2018open, saito2020universal, fu2020learning, bucci2020effectiveness}. 
% 
At a high level, most OSDA methods perform two steps: 
(i) align source and target representation
for previously seen classes; and (ii) train a 
discrimination to reject 
novel class from previously seen classes. 
The second step typically uses 
novelty detection heuristics
to identify  novel samples.
% to identify novel examples.

\textbf{PU Learning {} {}} 
\update{Positive and Unlabeled (PU) learning 
is the base case of OSLS}.
Here, we observe labeled data a single source class  
and unlabeled target data contains 
data from both the novel class and the source class. 
In PU learning, our goals are: 
(i) Mixture Proportion Estimation (MPE), i.e., 
determining the fraction of previously seen class 
in target ; and (ii) PU classification, 
i.e., learning to discriminate between
the novel and the positive (source) class.
Several classical methods were proposed 
for both MPE~\citep{elkan2008learning,du2014class,scott2015rate,jain2016nonparametric,bekker2018estimating,bekker2020learning} 
and classification~\citep{elkan2008learning, du2014analysis,du2015convex}. 
However, classical MPE methods
do not scale to high-dimensional settings~\citep{ramaswamy2016mixture}. 
% or yield estimators whose accuracy depends 
% on restrictive conditions~\citep{du2014class,scott2015rate}
More recent methods alleviate these issues
by operating in classifier output space~\citep{garg2021PUlearning, ivanov2019dedpul}. 
For classification, traditional methods fail 
when deployed with models classes with high capacity
due to their capacity of fitting random labels~\citep{zhang2016understanding}. 
Recent methods~\citep{garg2021PUlearning, kiryo2017positive, chen2020self}, 
avoid over-fitting by employing regularization 
or self-training techniques.

% By contrast, 

% OSLS unifies label shift estimation/classification and PU learning. 
% 
% Instead of introducing out-of-support examples 
% from both previously seen classes and 
% Notably, in OSLS, the previously seen classes can shift in prevalence 
% but the class conditionals $p(x|y)$ do not shift. 
% the novel class as typically done in OSDA setup, 
% in OSLS, we only observe out-of-support examples 
% for the novel class. 
% Thus, unlike OSDA where out-of-support examples
% Thus in OSLS, out-of-support examples 
% must belong to the novel class.
% may belong to either previously seen classes or novel classes,

% \todosg{say that it is unexplored and we are the first deep learning}

\textbf{Other related work {} {}}
% 
% In contrast to the OSDA problem, 
A separate line of work looks at the problem 
of Out-Of-Distribution (OOD) detection
\citep{hendrycks2016baseline,geifman2017selective,lakshminarayanan2016simple, jiang2018trust, ovadia2019can, zhang2020hybrid}. 
Here, the goal is to identify novel examples, 
i.e., samples that lie out of the support of training distribution. 
The main different between OOD detection and OSDA 
is that in OOD detection we do not have access to 
unlabeled data containing a novel class. 
% 
Recently, \citet{cao2021open} proposed 
open-world semi-supervised learning,
where the task is to not only identify 
novel classes in target but also to separate out different 
novel classes in an unsupervised manner. 

\update{Our work takes a step back 
from the hopelessly general OSDA setup,
introducing OSLS, a well-posed OSDA setting
where the sought-after parameters can be identified.}

% 
% v0
% 


% \textbf{(Closed Set) Domain Adaptation (DA) {} {}}
% Under DA, our goal is 
% to adapt a classifier trained on source data 
% to target data from which we only observe unlabeled examples. 
% % In domain adaptation 
% DA is classically explored 
% under two distribution shift scenarios~\citep{storkey2009training}: 
% (i) Covariate shift~\citep{zhang2013domain,zadrozny2004learning,cortes2010learning,cortes2014domain,gretton2009covariate}
% where $p(y|x)$ remains invariant
% among source and target; and 
% (ii) Label shift~\citep{saerens2002adjusting, lipton2018detecting, azizzadenesheli2019regularized, alexandari2019adapting, garg2020labelshift, zhang2020coping} where $p(x|y)$
% %doesn't change % from 
% is shared across source and target.
% % 
% \citet{scholkopf2012causal} illustrated
% how covariate shift and label shift
% correspond to causal and anti-causal prediction,
% respectively.
% % 
% As in these settings, 
% most of the theoretical 
% analysis requires 
% source distribution 
% cover the target support~\citep{ben2010impossibility}. 
% % 
% % Notably, \citet{ben2010theory} 
% % leverages hypothesis 
% % capacity constraints
% % to enable generalization to 
% % out-of-support samples. 
% % 
% However, recent empirically work in 
% DA~\citep{long2015learning,long2017deep, sun2016deep, sun2017correlation, zhang2019bridging, zhang2018collaborative, ganin2016domain, sohn2020fixmatch}     
% focuses on settings 
% motivated by benchmark datasets
% (e.g., WILDS~\citep{ sagawa2021extending, wilds2021}, 
% Office-31~\citep{saenko2010adapting}
% OfficeHome~\citep{venkateswara2017deep}, 
% DomainNet~\citep{peng2019moment}) 
% where the assumptions of
% contained support 
% are violated. 
% Instead, they rely 
% on under-specified 
% semantic equivalence
% assumptions between domains. 
% % Some methods 
% Despite access to unlabeled data 
% and careful hyperparameter tuning, 
% these popular empirical methods  
% often do not improve over 
% standard empirical risk minimization
% on source data alone for practical, 
% and importantly, previously unseen
% datasets~\citep{sagawa2021extending}.  




 
% \textbf{Open Set Domain Adaptation (OSDA) {} {}} 
% OSDA~\citep{panareda2017open, bendale2015towards, 6365193}
% extends DA problem where along with distribution 
% shift among previously seen classes, we may observe a
% novel class in the target data. 
% In DA literature, this setting is also known as
% universal domain adaptation~\citep{you2019universal, saito2020universal}. 
% Instead of making precise assumptions 
% on the nature of shift between source 
% and target, OSDA literature is primarily governed by 
% semi-synthetic problems on benchmark DA datasets
% (e.g. DomainNet, Office-31 and OfficeHome). 
% Numerous approaches have been 
% proposed for OSDA~\citep{baktashmotlagh2018learning, cao2019learning, tan2019weakly, lian2019known, you2019universal, saito2018open, saito2020universal, fu2020learning, bucci2020effectiveness}. 
% % 
% From a high level, OSDA methods perform two steps: 
% (i) align source and target representation
% for previously seen classes; and (ii) train a 
% domain discrimination classifier to reject 
% novel class from previously seen classes. 
% Second step involves novelty 
% detection heuristics to identify novel examples.
% A standard heuristic, typically 
% employed in practice, involves thresholding uncertainty  
% estimates based on classifier prediction, 
% e.g., prediction entropy, maximum confidence 
% or disagreement between  source classifiers~\citep{you2019universal,fu2020learning,tan2019weakly,saito2020universal}. 
% However, these hueristics often rely on carefully 
% tuned hyperparameter which may not transfer 
% across different dataset and different proportion of 
% novel classes. 

% \textbf{PU Learning {} {}} 
% Positive and Unlabeled (PU) 
% learning is the base case 
% of OSDA. Here, we observe labeled data a single 
% source class  
% and unlabeled target data contains 
% data from both the novel class and the source class. 
% In PU learning, our goals are: 
% (i) Mixture Proportion Estimation (MPE), i.e., 
% determining the fraction of previously seen class 
% in target domain; and (ii) PU classification, i.e., 
% learning to discriminate
% novel and the source class.
% Traditionally, several methods have been proposed for 
% both MPE~\citep{elkan2008learning,du2014class,scott2015rate,ramaswamy2016mixture,jain2016nonparametric,bekker2018estimating,bekker2020learning} 
% and classification~\citep{elkan2008learning, du2014analysis,du2015convex}. 
% However, classical MPE methods
% do not scale to high-dimensional settings~\citep{ramaswamy2016mixture}
% or yield estimators whose accuracy depends 
% on restrictive conditions~\citep{du2014class,scott2015rate}
% More recent methods, alleviate these issues by 
% leverage blackbox classifiers~\citep{garg2021PUlearning, ivanov2019dedpul}. 
% For classification, traditional methods fail 
% when deployed with models classes with high capacity
% due to their capacity of fitting random labels~\citep{zhang2016understanding}. 
% Recent methods~\citep{garg2021PUlearning, kiryo2017positive, chen2020self}, 
% avoid overfitting issues by employing regularization or 
% self-training techniques.

% Contrastingly, in our work, we take a step back from a typical
% OSDA setup and propose a simple OSLS setting which 
% unifies label shift scenario and PU learning. 
% % 
% Instead of introducing out-of-support examples 
% from both previously seen classes and 
% the novel class as typically done in OSDA setup, 
% in OSLS, we only observe out-of-support examples 
% for the novel class. \todosg{say that it is unexplored and we are the first deep learning}




% \textbf{Other related work {} {}}
% % 
% In contrast to the OSDA problem, 
% a separate line of work 
% looks at the problem of Out-Of-Distribution (OOD) 
% or anomaly detection~\citep{hendrycks2016baseline,geifman2017selective, 
% lakshminarayanan2016simple, jiang2018trust, ovadia2019can, zhang2020hybrid, vaze2021open}. 
% Here, the goal is to identify previously unseen
% examples, i.e., samples out of the 
% support of training distribution. 
% The main different between OOD detection and OSDA 
% is that in OOD detection we do not have access to 
% unlabeled data containing a novel class. 
% % 
% Recently, \citet{cao2021open} 
% proposed open-world semi-supervised learning 
% where the task is to not only identify 
% novel classes in target but also to 
% separate out different 
% novel classes in an unsupervised manner. 


% % Note that unlike 
% % domain generalization, 





% % https://github.com/thuml/Calibrated-Multiple-Uncertainties/tree/master/current -- tweeked 2_0 for different datasets 
% % https://github.com/VisionLearningGroup/DANCE

==> Open set label shift (NeurIPS 2022)/sections/03_2_reduction.tex <==
Under the strong positivity condition, 
the OSLS problem can be broken down
into $k$ PU problems as follows: 
% 
By treating a given source class $y_j \in \out_s$
as \emph{positive} and grouping
all other classes together as \emph{negative}
we observe that the unlabeled target data 
is then a mixture of data from 
the positive and negative classes.
This yields a PU learning problem 
and the corresponding mixture proportion 
is the 
fraction $\pt(y = j)$ (proportion of class $y_j$) among the target data.
By iterating this process for all source classes,
we can solve for the entire target label marginal $\pt(y)$.
Thus, OSLS reduces to $k$ instances of PU learning problem. 
Formally, note that $\pt(x)$ can be written as:
\begin{align}
\pt(x) = \pt(y=j) \ps(x|y = j) + \left(1- \pt(y=j)\right) \left(\sum\nolimits_{ i \in \out \setminus \{j\}} \mfrac{\pt(y = i)}{ 1- \pt(y = j)} \ps(x|y = i)\right) \label{eq:reduction}\,, 
\end{align}
individually for all $j \in \out_s$. 
By repeating this reduction for all classes,
we obtain $k$ separate PU learning problems. 
Hence, a natural choice is to leverage 
this structure and solve $k$ PU problems
to solve the original OSLS problem. 
\update{In particular, for each class $j \in \out_s$, 
we can first estimate its prevalence $\hat \pt(y = j)$
in the unlabeled target. 
Then the target marginal for the novel class is given by 
$\smash{\hat \pt( y = k+1) = 1 - \sum_{i=1}^k \hat \pt (y = i) }$.}
Similarly, for classification,
we can train $k$ PU learning classifiers $f_i$,
where $f_i$ is trained to classify a source class $i$ 
versus others in target. 
An example is classified as belonging to the class
$y=k+1$, if it rejected by all classifiers $f_i$ as other in target. 
We explain this procedure more formally in \appref{subsec:reduction}. 
% Note that this reduction of OSLS problem to $k$ PU problems
% is not applicable under separability. \todosg{elaborate why?}


This reduction has been mentioned in past work
\citep{sanderson2014class, xu2017multi}. 
% as extension of PU learning problem to $k$
% classes. 
However, to the best of our knowledge, 
no previous work has empirically investigated 
both classification and target label marginal 
estimation jointly. %, even under strong positivity.
% However, authors in \citep{sanderson2014class, xu2017multi} 
% do not explore both the tasks jointly for the OSLS problem. 
\citet{sanderson2014class} 
focuses only on target marginal estimation 
for 
% low-dimensional 
tabular datasets 
and \citet{xu2017multi} assumes that 
the target marginal is known and only 
trains $k$ separate PU classifiers. 

In our work, 
% has also not been evaluated 
% rigorously (if at all) 
% 
we perform the first large scale experiments 
to evaluate efficacy of the reduction 
of the OSLS problem to $k$-PU problems.
With plugin state-of-the-art PU learning algorithms, 
% that scale 
% to practical deep learning. 
% 
we observe that this naive reduction doesn't scale 
to datasets with large number of classes
because of error accumulation in each 
of the $k$ MPEs 
and $k$ one-versus-other PU classifiers.
% (we elaborate in \secref{sec:framework}). 
To mitigate the error accumulation problem, 
we propose the PULSE framework in the next section. 

% 
% v0.5
% 

% Under the strong positivity condition, 
% the OSLS problem can be broken down
% into $k$ PU problems as follows: 
% % 
% By treating a given source class $y_j \in \out_s$
% as \emph{positive} and grouping
% all other classes together as \emph{negative}
% we observe that the unlabeled target data 
% is then a mixture of data from 
% the positive and negative classes.
% This yields a PU learning problem 
% and the corresponding mixture proportion
% gives the fraction $\alpha_j$ of class $y_j$ among the target data.
% By iterating this process for all source classes,
% we can solve for the entire target label marginal $\pt(y)$.
% Thus OSLS reduces to $k$ instances of PU learning problem. 
% Formally, note that $\pt(x)$ can be written as:
% \begin{align}
% \pt(x) = \ps(y=j) \ps(x|y = j) + \left(1- \ps(y=j)\right) \left(\sum\nolimits_{ i \in \out \setminus \{j\}} \mfrac{\ps(y = i)}{ 1- \ps(y = j)} \ps(x|y = i)\right) \label{eq:reduction}\,, 
% \end{align}
% individually for all $j \in \out_s$. 
% By repeating this reduction for all classes,
% we obtain $k$ separate PU learning problems. 
% Hence, a natural choice is to leverage 
% this structure and solve $k$ PU problems
% to solve the original OSLS problem. 
% In particular, for each class $j \in \out_s$, 
% we can first estimate its prevalence $\hat \alpha_j$
% in the unlabeled target. Then the target marginal for the novel 
% class is given by 
% $\hat \alpha_{k+1} = 1 - \sum_{i=1}^k \hat \alpha_i$. 
% Similarly, for classification, we can train 
% $k$ PU learning classifiers $f_i$, where 
% $f_i$ is trained to classify a source class $i$ 
% versus others in target. 
% An example is classified as belonging to the class
% $y=k+1$, if it rejected by all classifiers $f_i$
% as other in target. We explain this procedure more formally in 
% \appref{subsec:reduction}. 
% Note that this reduction of OSLS problem to $k$ 
% PU problems is not applicable under separability. \todosg{elaborate why?}


% This reduction has been dabbled in past work
% \citep{sanderson2014class, xu2017multi} 
% as extension of PU learning problem to $k$
% classes. However, to the best of our knowledge, 
% no previous work has empirically investigated 
% both classification and target label marginal 
% estimation jointly even under strong positivity.
% % However, authors in \citep{sanderson2014class, xu2017multi} 
% % do not explore both the tasks jointly for the OSLS problem. 
% \citet{sanderson2014class} 
% focuses only on target marginal estimation 
% for low-dimensional tabular datasets 
% and \citet{xu2017multi} assumes that 
% the target marginal is known and only 
% trains $k$ separate PU classifiers. 

% In our work, 
% % has also not been evaluated 
% % rigorously (if at all) 
% % 
% we perform first large
% scale experiments 
% to evaluate efficacy of the 
% naive reduction of OSLS problem to $k$-PU problems.
% Even with plugin state-of-the-art PU learning 
% algorithms, 
% % that scale 
% % to practical deep learning. 
% % 
% we observe that this 
% naive reduction doesn't scale 
% to practical deep learning datasets
% because of error accumulation in each of $k$
% mixture proportion estimates and
% $k$ one-versus-other PU classifiers
% (we elaborate this in
% \secref{sec:framework}). 
% To alleviate the error accumulation 
% problem, we propose 
% PULSE framework in the next section. 

==> Open set label shift (NeurIPS 2022)/sections/03_setup.tex <==
% 
% v1
% 

\textbf{Notation {} {}} 
% By $\enorm{\cdot}$ and $\inner{\cdot}{\cdot}$,
% we denote the Euclidean norm and inner product,
% respectively.
For a vector $v\in \Real^d$, 
we use $v_j$ to denote its $j^\text{th}$ entry, 
and for an event $E$, we let $\indict{E}$ 
denote the binary indicator of the event.
By $\abs{A}$, we denote the cardinality of set $A$.  

Let $\inpt \in \Real^d $ be the input space 
and $\out = \{ 1,2, \ldots, k+1\}$ be the output space
for multiclass classification.
Let $\ProbS$ and $\ProbT$ be the 
source and target distributions and 
let $\ps$ and $\pt$ denote the corresponding 
% probability density function or probability mass function. 
probability density (or mass) functions. 
% 
By $\mathbb{E}_s$ and $\mathbb{E}_t$, 
we denote expectations over 
the source and target distributions.
We assume that we are given a loss function 
$\lossell: \Delta^{k} \times \out \to \Real $,
such that $\ell(z, y)$ is the loss incurred 
by predicting $z$ when the true label is $y$. 
Unless specified otherwise,
we assume that $\ell$ is the cross entropy loss. 
% 
As in standard unsupervised domain adaptation, 
we are given independently and identically distributed (iid) 
samples from labeled source data 
$\{(\x_1,y_1), (\x_2, y_2), \ldots , (\x_n, y_n)\}\sim \ProbS^n$ 
and iid samples from unlabeled target data
$\{\x_{n+1}, \x_{n+2}, \ldots, \x_{n+m}\}\sim \ProbT^m$.  
% 

Before formally introducing OSLS, we describe 
label shift and PU learning settings. 
Under label shift, we observe data 
from $k$ classes in both source 
and target where the conditional 
distribution remain invariant 
(i.e., $p_s(x|y) = p_t(x|y)$ 
for all classes $y \in [1,k]$) 
but the target label marginal  
may change (i.e., $p_t(y) \ne p_s(y)$). 
Additionally, for all classes 
% which may be observed in target 
% we have a non-zero support 
% for those 
in source have a non-zero support , i.e., 
for all $y\in [1, k]$, $p_s(y) \ge c$, where $c > 0$. 
% 
Under PU learning, we possess labeled source data 
from a positive class and unlabeled target data 
from a mixture of positive and negative class
with a goal of learning a positive-versus-negative classifier
on target. 
%  
We now introduce the OSLS setting:

% \todosg{Not sure if definition is better?}



\begin{definition}[Open set label shift]
% Assume that the source contains $k$ classes. 
Define $\out_t = \out$ and 
$\out_s = \out \setminus \{k+1\}$. 
% 
Under OSLS, the label distribution among 
source classes $\out_s$ may change
but the class conditional $p(x|y)$ 
for those classes remain invariant 
between source and target, 
and the target domain may contain a novel class, i.e., 
% $\ps(y = k+1) = 0$ and $\ps(x|y = j) = \pt(x|y=j)$
% for all $j \in \out \setminus \{k+1\}$.
\begin{align}
    \ps(x|y = j) = \pt(x|y=j) \quad \forall j \in \out_s \qquad \text{and} \qquad \ps(y = k+1) = 0 \,. \label{eq:OSLS}
\end{align}
% Additionally, we assume
Additionally, we have non-zero support 
for all $k$ (previously-seen) labels 
in the source distribution, 
i.e., for all $y \in \out_s$, 
$\ps(y) \ge c$ for some $c > 0$. 
\end{definition}

Note that the label shift and PU learning problems
can be obtained as special cases of OSLS.  
When no novel class is observed in target 
(i.e., when $p_t(y = k+1) = 0$),
we recover the label shift problem,
and when we observe only one class in source 
(i.e., when $k=1$), 
the OSLS problem reduces to PU learning.
% We formally define label shift and PU learning 
% problems in \appref{sec:prelims}.
% As 
% 
Under OSLS, our goal naturally breaks 
down into two tasks: 
(i) estimate the target label marginal $p_t(y)$ 
for each class $y \in \out$; 
(ii) 
% given an estimate of $p_t(y)$, 
train a classifier $f: \inpt \to \Delta^k$ 
to approximate $p_t(y|x)$. 
% for the target domain.  
% 
% We evaluate classifier performance by 0-1 

% 
% Next, we propose PULSE frameworl


% 
% v0
% 

% \textbf{Notation {} {}} By $\enorm{\cdot}$ and $\inner{\cdot}{\cdot}$,
% we denote the Euclidean norm and inner product, respectively.
% For a vector $v\in \Real^d$, 
% we use $v_j$ to denote its $j^\text{th}$ entry, 
% and for an event $E$, we let $\indict{E}$ 
% denote the binary indicator of the event.
% By $\abs{A}$, we denote the cardinality of set $A$.  
% % Let $\Prob : \inpt\times\out \to [0,1]$
% % be the underlying joint distribution 
% % and let $p$ denote its corresponding density.

% Suppose $\inpt \in \Real^d $ be the input space 
% and $\out = \{ 1,2, \ldots, k+1\}$ be the output space
% for multiclass classification.
% Let $\ProbS$ and $\ProbT$ be the 
% source and target distributions and 
% let $\ps$ and $\pt$ denote the corresponding 
% % probability density function or probability mass function. 
% probability density (or mass) functions. 
% % 
% With $\mathbb{E}_s$ and $\mathbb{E}_t$, we denote expectations 
% over the source and target distributions.
% % 
% We assume that we are given a loss function 
% $\lossell: \Delta^{k} \times \out \to \Real $,
% such that $\ell(z, y)$ is the loss incurred 
% by predicting $z$ when the true label is $y$. 
% Unless specified otherwise, we assume $\ell$
% is cross entropy loss. 
% % 
% As in standard unsupervised domain adaptation, 
% we are given independently and identically distributed (iid) 
% samples from 
% labeled source data 
% $\{(\x_1,y_1), (\x_2, y_2), \ldots , (\x_n, y_n)\}\sim \ProbS^n$ 
% and iid samples from 
% unlabeled target data $\{\x_{n+1}, \x_{n+2}, \ldots, \x_{n+m}\}\sim \ProbT^m$.  
% % 

% Before formally introducing 
% OSLS setting, we describe
% label shift and PU learning
% settings. 
% Under label shift, 
% we observe data from $k$ classes in
% both source and target where 
% the conditional 
% distribution remain invariant 
% (i.e., $p_s(x|y) = p_t(x|y)$ 
% for all classes $y \in [1,k]$) 
% but the target label marginal  
% may change (i.e., $p_t(y) \ne p_s(y)$). 
% Additionally, for all classes which may be
% observed in target we have a non-zero support 
% for those in source, i.e., for all $y\in [1, k]$,  
% $p_s(y) \ge c$ where $c > 0$. 
% % 
% Under PU learning, we possess labeled source data from
% a positive class and unlabeled target data 
% from a mixture of positive and negative class
% with a goal of learning a positive-versus-negative classifier on 
% target. 
% %  
% We can now introduce the OSLS setting:

% % \todosg{Not sure if definition is better?}



% \begin{definition}[Open set label shift]
% % Assume that the source contains $k$ classes. 
% Define $\out_t = \out$ and as $\out_s = \out \setminus \{k+1\}$. 
% % 
% Under OSLS, the label distribution among source classes $\out_s$ may change but the class conditional $p(x|y)$ for those classes remain 
% invariant between source and target, 
% and the target domain may contain a novel class, i.e., 
% % $\ps(y = k+1) = 0$ and $\ps(x|y = j) = \pt(x|y=j)$
% % for all $j \in \out \setminus \{k+1\}$.
% \begin{align}
%     \ps(x|y = j) = \pt(x|y=j) \quad \forall j \in \out_s \qquad \text{and} \qquad \ps(y = k+1) = 0 \,. \label{eq:OSLS}
% \end{align}
% Additionally, assume non-zero support for 
% all the $k$ labels in the source distribution, i.e., for all $y \in \out_s$, 
% $\ps(y) \ge c$ for some $c > 0$. 
% \end{definition}

% Note that the label shift and PU learning problem
% can be obtained as special cases of OSLS.  
% When no novel class 
% is observed in target (i.e., when $p_t(y = k+1) = 0$),
% we recover the label shift problem, and 
% when we observe only one class in source (i.e., when $k=1$), 
% the OSLS problem reduces to PU learning.
% % We formally define label shift and PU learning 
% % problems in \appref{sec:prelims}.
% % As 
% % 
% Under OSLS,  
% our goal naturally breaks 
% down into two tasks: (i) estimate the 
% target label marginal $p_t(y)$ for each class $y \in \out$; 
% (ii) given an estimate of $p_t(y)$, train a 
% classifier $f: \inpt \to \Delta^k$ 
% to approximate $p_t(y|x)$. 
% % for the target domain.  
% % 
% % We evaluate classifier performance by 0-1 

% % 
% % Next, we propose PULSE frameworl



==> Open set label shift (NeurIPS 2022)/sections/04_identifiability.tex <==
We now introduce conditions for OSLS,
under which the solution is identifiable. 
Throughout the section, 
we will assume access to population 
distribution for labeled source data and unlabeled target data, 
i.e., $p_s(x,y)$ and $p_t(x)$ is given. To keep
the discussion simple, we assume finite input domain $\inpt$
which can then be relaxed to continuous inputs. 
We relegate proofs to \appref{sec:proof_identi_app}. 
% Our results can be easily extended to continuous 
% input domains. 

We first make a connection between target 
label marginal $\pt(y)$ estimation 
and learning the target classifier $\pt(y|x)$
showing that recovering $\pt(y)$ is 
enough to identify $p_t(y|x)$. 
\update{In population, given access to $p_t(y)$, the 
class conditional $\pt(x|y=k+1)$ can be 
obtained in closed form as $\nicefrac{\left(\pt(x) - \sum_{j=1}^k \pt(y=j) \ps(x|y=j)\right)}{p_t(y = k+1)}$.} 
We can then apply Bayes rule to obtain $\pt(y|x)$.  
Henceforth, we will focus our discussion on identifiability 
of $\pt(y)$ which implies identifiability of $p_t(y|x)$. 
% 
% 
In following proposition, we present \emph{weak positivity},
a necessary condition for $p_t(y)$ to be identifiable. 
% For ease, 
% we denote $\out_t = \out$ and $\out_s = \out \setminus \{k+1\}$ 
% 
%
\begin{restatable}[Necessary conditions]{reprop}{necessary} \label{prop:necessary}
Assume $p_t(y) > 0$ for all $y\in \out_t$. Then 
$p_t(y)$ is identified only if $\pt(x|y=k+1)$ and 
$\ps(x|y)$ for all $y\in \out_s$ satisfy weak positivity, i.e., there must  
exists a subdomain $X_\wpos \subset X$ such that:
\begin{enumerate}[(i)]
  \setlength{\itemsep}{3pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
    \item  $\pt(X_\wpos | y = k+1) = 0$; and 
    \item the matrix $\left[\ps(x|y)\right]_{x\in X_\wpos, y\in \out_s}$ is full column-rank. 
\end{enumerate}
\end{restatable}

% 
% 
Intuitively, \propref{prop:necessary} states 
that if the target marginal doesn't lie
on the vertex of the simplex $\Delta^k$,
then their must exist a subdomain $X_\wpos$ 
where the support of novel class is zero 
and within $X_\wpos$, 
$\pt(y)$ for source classes is identifiable. 
While it may seem that existence of 
a subdomain $X_\wpos$ is enough, 
we show that for the OSLS problem, 
existence doesn't imply uniqueness. 
In \appref{subsec:counter}, 
we construct an example,
where the weak positivity condition is not sufficient. 
% Since we only have access to $p_s(x,y)$, 
In that example, we show that there can 
exist two subdomains $X_\wpos$ 
and $X_\wpos^\prime$ satisfying weak positivity, 
both of which lead to separate solutions for $\pt(y)$.
% 
Next, we extend weak positivity to 
two stronger conditions, 
either of which (alone) implies identifiability. 
% 
\begin{restatable}[Sufficient conditions]{reprop}{sufficient} \label{prop:sufficiency}
The target marginal $p_t(y)$ is identified 
if for all $y\in \out \setminus \{k+1\}$, 
$\pt(x|y=k+1)$ and  $\ps(x|y)$ 
satisfy either:
\begin{enumerate}[(i)]
  \setlength{\itemsep}{3pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
    \item Strong positivity, i.e.,
there exists $X_\spos \subset \inpt$ 
such that $p_t(X_\spos| y= k+1) = 0$ 
and the matrix $\left[\ps(x|y)\right]_{x\in X_\spos, y\in \out_s}$
is full-rank and diagonal; or
    \item Separability, i.e., there exists $X_\sep \subset \inpt$,
such that $p_t(X_\sep | y= k+1 ) = 0\,$, $p_s(X_\sep) = 1\,,$ 
and the matrix $\left[\ps(x|y)\right]_{x\in X_\sep, y\in \out_s}$ 
is full column-rank. 
\end{enumerate}
\end{restatable}
% 
Strong positivity generalizes the irreducibility 
condition~\citep{blanchard2010semi}, 
which is sufficient for identifiability under PU learning,
to $k$ PU learning problems. 
% 
Note that while the two conditions 
in \propref{prop:sufficiency} overlap, 
they cover independent set of OSLS problems.  
% 
Informally, strong positivity extends weak positivity 
by making an additional assumption that the matrix 
formed by $p(x|y)$ on inputs in $X_\wpos$ is diagonal 
and the separability assumption
extends the weak positivity condition 
to the full input domain of source classes
instead of just $X_\wpos$. 
Both of these conditions identify 
a support region of $\inpt$ 
which purely belongs to source classes 
where we can either individually estimate 
the proportion of each source classes 
(i.e., under strong positivity) 
or jointly estimate the proportion 
(i.e., under separability). 

% \todosg{Think if want to add the exponentially hard to check condition here which is necessary and sufficient?}
% 


To extend our identifiability conditions 
for continuous distributions, 
the linear independence 
conditions on the matrix 
$\left[\ps(x|y)\right]_{x\in X_\sep, y\in \out_s}$
has the undesirable property of being 
sensitive to changes on sets of measure zero.
We may introduce stronger notions 
of linear independence as in Lemma 1 
of \citet{garg2020labelshift}.
We discuss this in \appref{subsec:extend_ident_continuos}.  


% \begin{itemize}
%     \item Necessary and sufficient conditions 
%     \item Explain what is necessary, explain what is sufficient
%     \item explain why necessary conditions are not enough. 
%     \item Give an algorithm that characterizes necessary and sufficient condition -- http://www.ece.umn.edu/~nikos/06630130.pdf
% \end{itemize}

==> Open set label shift (NeurIPS 2022)/sections/05_approach.tex <==

We begin with presenting our framework for OSLS problem 
under strong positivity condition. 
% and 
% then discuss its extension under separability condition. 
First, we explain the structure of OSLS 
that we leverage in PULSE framework
and then elaborate design decisions 
we make
% on how 
to exploit the identified structure.

% \todosg{some more to add as motivation or why it is hard?}

\paragraph{Overview of PULSE framework}
Rather than simply dividing each 
OSLS instance into $k$ PU problems, 
we exploit the joint structure 
of the problem to obtain a \emph{single} PU learning problem. 
% we exploit a different structure of the problem. 
% We begin with 
To begin, we note that if only 
we could apply a
\emph{label shift correction}
to source, i.e.,
re-sample source classes 
according to their relative proportion
in the target data,
then we could subsequently consider 
the unlabeled target data 
as a mixture of (i)
the (reweighted) source distribution;
and (ii) the novel class distribution 
(i.e., $p_t(x|y=k+1)$). 
\update{Formally, we have 
\begin{align*}
    p_t(x) = \sum_{j \in \out_t} p_t(y=j) & p_t(x|y=j)  = 
    \sum_{j \in \out_s} \mfrac{p_t(y=j)}{p_s(y=j)} p_s(x, y=j) + p_t(x|y=k+1) p_t(y=k+1) \\
    &= (1- p_t(y=k+1)) p_s^\prime(x) + p_t(y=k+1) p_t(x|y=k+1)\,, \numberthis \label{eq:label_shift_corr}
\end{align*}
where $p_s^\prime(x)$ is the label-shift-corrected source distribution, 
i.e., $p_s^\prime(x) = \sum_{j \in \out_s} w(j) p_s(x,y=j)$,
where $w(j) = {\left(\nicefrac{p_t(y=j)}{\sum_k p_t(y=k)}\right)}/{p_s(y=j)}$ 
for all $j \in \out_s$. 
Intuitively, $p_t^\prime(j) = \nicefrac{p_t(y=j)}{\sum_k p_t(y=k)}$ is
re-normalized label distribution in target 
among source classes 
and $w(j)$'s are the importance weights.} %ratios. 
% For ease of notation, we refer $p_t^\prime(y)$ as the re-normalized label distribution 
% among previously seen classes, i.e., 
% $p_t^\prime(y = j) = {p_t(y=j)}/{\sum_k p_t(y=k)}$. 
% 
Hence, after applying a label shift correction
to the source distribution $p_s^\prime(x)$, 
we have reduced the OSLS problem 
to a \emph{single} PU learning problem,
where $p_s^\prime(x)$ plays the part 
of the positive distribution and $p_t(x| y=k+1)$ acts
as negative distribution with mixture coefficients
$1 - p_t(y=k+1)$ and $p_t(y=k+1)$ respectively. 
\update{We now discuss our methods (i) to estimate 
the importance ratios $w(y)$; 
and (ii) to tackle the PU learning instance obtained from OSLS.  
% 
}


\paragraph{Label shift correction: Target marginal estimation among source classes} While traditional methods for estimating label shift 
breakdown in high dimensional settings~\citep{zhang2013domain}, 
recent methods exploit black-box classifiers
to avoid the curse of dimensionality~\citep{lipton2018detecting, azizzadenesheli2019regularized, alexandari2019adapting}. 
However, these recent techniques
require overlapping label distributions, 
and a direct application would require
demarcation of samples from $p^\prime_s(x)$ \update{sub-population} 
in target, creating a cyclic dependency. 
% 
\update{Instead, to estimate the relative proportion of previously seen classes in target, we leverage the $k$ PU reduction described in \secref{sec:reduction} with two crucial distinctions. First, we normalize the obtained estimates of fraction previously seen classes to obtain the relative proportions in $\ps^\prime(y)$. In particular, we do not leverage the estimates of previously seen class proportions in target to directly estimate the proportion of novel class which avoids issues due to error accumulation. 
% 
Second, we exploit a $k$-way source classifier $f_s$ trained on labeled source data instead of training $k$ one-versus-other PU classifiers. }
% 
\update{
% To estimate the proportion of previously seen classes, 
We tailor the recently proposed 
Best Bin Estimation (BBE) 
technique from \citet{garg2021PUlearning}. 
% Given positive and unlabeled data, 
% BBE estimates the fraction of positives in unlabeled 
% by leveraging a black-box classifier. 
% 
We describe the modified BBE procedure in 
\appref{sec:OSLS_framework_app} (\algoref{alg:BBE}). 
% 
After estimating the relative fraction 
of source classes in target (i.e., $\wh p_t^\prime(j) =\nicefrac{ \wh p_t(y=j)}{\sum_{k\in \out_s} \wh p_t(y=k)}$ for all $j \in \out_s$), 
we re-sample the source data according to $\wh p_t^\prime(y)$
to mimic samples from distribution $p_s^\prime(x)$. 
}

\begin{algorithm}[t!]
  \caption{Positive and Unlabeled learning post Label Shift Estimation (PULSE) framework}
  \label{alg:PULSE}
  \begin{algorithmic}[1]
  \INPUT: Labeled source data $\{{\bf X}^S, {\bf y}^S\}$ and unlabeled target samples ${\bf X}^T$. 
    \STATE Randomly split data into training $\{{\bf X}^S_1, {\bf y}^S_1\}$, ${\bf X}^T_1$ and hold out partition $\{{\bf X}^S_2, {\bf y}^S_2\}$, ${\bf X}^T_2$.
    \STATE Train a source classifier $f_s$ on labeled source data $\{{\bf X}^S_1, {\bf y}^S_1\}$.
    \STATE \update{Estimate label shift $\wh p^\prime_t(y = j) = \mfrac{\wh p_t(y=j)}{\sum_{k\in \out_s} \wh p_t(y=k)}$ using \algoref{alg:BBE}} and hence importance ratios $\wh w(j)$ among source classes $j \in \out_s$. 
    \STATE Re-sample training source data according to label distribution  $\wh p^\prime_t$ to get $\{ \widetilde{\bf X}^S_1, \widetilde{\bf y}^S_1\}$ and $\{ \widetilde{\bf X}^S_2, \widetilde{\bf y}^S_2\}$. 
    \STATE Using \algoref{alg:CVIR}, train a discriminator $f_d$ and estimate novel class fraction $\wh p_t(y=k+1)$. 
    \STATE Assign $[f_t(x)]_j = (f_d(x)) \mfrac{\wh w(j) \cdot [f_s(x)]_j}{\sum_{k\in \out_s} \wh w(k) \cdot [f_s(x)]_k} $ for all $j \in \out_s$ and $[f_t(x)]_{k+1} = 1 - f_d(x)$. And for all $j \in \out_s$, assign $\wh p_t(y = j) = (1-\wh p_t(y=k+1))\cdot \wh p_t^\prime(y = j)$. 
  \OUTPUT: Target marginal estimate $\wh p_t \in \Delta^k$ and target classifier $f_t (\cdot) \in \Delta^k$.  
\end{algorithmic}
\end{algorithm}



\paragraph{PU Learning: Separating the novel class from previously seen classes}
After obtaining a PU learning problem instance, 
we resort to PU learning techniques to 
(i) estimate the fraction of novel class $p_t(y=k+1)$; 
and (ii) learn a binary classifier $f_d(x)$ to discriminate 
between label shift corrected source $p_s^\prime(x)$
and novel class $p_t(x|y=k+1)$. 
% 
\update{
% For ease of exposition, we assume that the sigmoid output $f_d(x)$ indicates the predicted probability of an example $x$ belonging to label shift corrected source $p_s^\prime(x)$.  
% 
With traditional methods for PU learning
involving domain discrimination, 
over-parameterized models can
memorize the positive instances 
in unlabeled,
assigning them confidently 
to the negative class,
which can severely hurt
generalization on PN 
data~\citep{kiryo2017positive, garg2021PUlearning}.
Rather, we employ Conditional 
Value Ignoring Risk (CVIR) loss
proposed in \citet{garg2021PUlearning} 
which was shown to outperform alternative 
approaches.
First, we estimate the proportion 
of novel class $\wh p_t(y=k+1)$ with BBE.
Next, given an estimate $\wh p_t(y=k+1)$,
CVIR objective discards
the highest loss 
$(1 - \wh p_t(y=k+1))$ fraction of examples
on each training epoch, removing the 
incentive to overfit to
the examples from $p_s^\prime(x)$. 
% In particular,  
% 
Consequently, we employ the 
iterative procedure that alternates between 
estimating the prevalence 
of novel class $\wh p_t(y=k+1)$ (with BBE) and 
minimizing the CVIR loss with estimated 
fraction of novel class. 
% 
We detail this procedure in \appref{sec:OSLS_framework_app} (\algoref{alg:CVIR}).  
}

\paragraph{Combining PU learning and label shift correction} 
Finally, to obtain a $(k+1)$-way classifier $f_t(x)$ on target 
we combine discriminator $f_d$ and  source classifier $f_s$
with importance-reweighted label shift correction. 
In particular,
for all $j \in \out_s$, $[f_t(x)]_j = (f_d(x)) \frac{w(j) \cdot [f_s(x)]_j}{\sum_{k\in \out_s} w(k) \cdot [f_s(x)]_k} $
and $[f_t(x)]_{k+1} = 1 - f_d(x)$. 
\update{Overall, our approach outlined in \algoref{alg:PULSE} proceeds
as follows:
% 
First, we estimate the label shift among
previously seen classes. 
% by leveraging 
% a source classifier $f_s$, 
Then we employ importance re-weighting of source 
data to formulate a single PU learning problem 
% between source and target
to estimate the fraction 
of novel class $\wh p_t(y=k+1)$ and 
to learn a discriminator $f_d$ 
for the novel class. Combining discriminator 
and label shift corrected source classifier
we get $(k+1)$-way target classifier. 
We analyse crucial steps in PULSE in 
\secref{sec:analysis}.} 
% \todosg{Finish this!}
% 


Our ideas for PULSE framework 
can be
extended to separability 
condition since   
\eqref{eq:label_shift_corr}
continues to hold. 
However, in our initial experiments,
we observe that techniques proposed 
under strong positivity were empirically 
stable and outperform methods
developed under separability.
This is intuitive for many benchmark datasets 
where it is natural to assume that 
for each class there exists a 
subdomain that only belongs to that class. 
% 
We describe this in more detail in \appref{subsec:pulse_separablity_app}. %\todosg{Re check this?}
% leave careful investigation for future work?


% Moreover, 
% We experimentally demonstrate the 
% failure of this naive reduction  
% in \secref{sec:exp}. 



% 
% v0
% 

% \begin{algorithm}[t!]
%   \caption{Positive and Unlabeled learning post Label Shift Estimation (PULSE) framework}
%   \label{alg:PULSE}
%   \begin{algorithmic}[1]
%   \INPUT: Labeled source data $\{\bf X^S, y^S\}$ and unlabeled target samples $\bf X^T$. 
%     \STATE Randomly split data into training $\{\bf{X}^S_1, \bf{y}^S_1\}$, $\bf{X}^T_1$ and hold out partition $\{\bf X^S_2, \bf y^S_2\}$, $\bf X^T_2$.
%     \STATE Train a source classifier $f_s$ on labeled source data $\{\bf{X}^S_1, \bf{y}^S_1\}$.
%     \STATE Estimate label shift $\wh p^\prime_t(j) = \mfrac{\wh p_t(y=j)}{\sum_{k\in \out_s} \wh p_t(y=k)}$ and hence importance ratios $\wh w(j)$ among source classes $j \in \out_s$ using \algoref{alg:BBE}. 
%     \STATE Re-sample training source data according to label distribution  $\wh p^\prime_t(j)$ to get $\{ \widetilde{\bf X}^S_1, \widetilde{\bf y}^S_1\}$. 
%     \STATE Using \algoref{alg:CVIR}, train a discriminator $f_d$ and estimate novel class fraction $\wh p_t(y=k+1)$. 
%     \STATE Assign $[f_t(x)]_j = (1 - f_d(x)) \mfrac{\wh w(j) \cdot [f_s(x)]_j}{\sum_{k\in \out_s} \wh w(k) \cdot [f_s(x)]_k} $ for all $j \in \out_s$ and $[f_t(x)]_{k+1} = f_d(x)$. And for all $j \in \out_s$, assign $\wh p_t(y = j) = (1-\wh p_t(y=k+1))\cdot \wh p_s^\prime(y = j)$. 
%   \OUTPUT: Target marginal estimate $\wh p_t \in \Delta^k$ and target classifier $f_t (\cdot) \in \Delta^k$.  
% \end{algorithmic}
% \end{algorithm}

% We present our framework for OSLS problem 
% under strong positivity condition and 
% then discuss its extension under separability condition. 
% First, we explain the structure of OSLS 
% that we leverage in PULSE framework
% and then elaborate design decisions 
% we make
% % on how 
% to exploit the identified structure. 

% % \todosg{some more to add as motivation or why it is hard?}

% Instead of dividing the OSLS
% into $k$ PU problems, we 
% exploit a different structure of the problem. 
% % We begin with 
% Noticing that after 
% \emph{label shift correction} 
% among previously seen classes 
% in the source domain, 
% we can consider unlabeled target data 
% as a mixture of label shift corrected 
% source distribution 
% (say $p_s^\prime(x)$) and novel 
% class distribution (i.e., $p_t(x|y=k+1)$). 
% Formally, we have 
% \begin{align*}
%     p_t(x) = \sum_{j \in \out_t} p_t(y=j) & p_t(x|y=j)  = 
%     \sum_{j \in \out_s} \mfrac{p_t(y=j)}{p_s(y=j)} p_s(x, y=j) + p_t(x|y=k+1) p_t(y=k+1) \\
%     &= (1- p_t(x|y=k+1)) p_s^\prime(x) + p_t(x|y=k+1) p_t(y=k+1)\,, \numberthis \label{eq:label_shift_corr}
% \end{align*}
% where $p_s^\prime(x)$ is the label shift corrected source distribution, i.e., 
% $p_s^\prime(x) = \sum_{j \in \out_s} w(j) p_s(x,y=j)$,
% where $w(j) = {\left(\nicefrac{p_t(y=j)}{\sum_k p_t(y=k)}\right)}/{p_s(y=j)}$ for all $j \in \out_s$. 
% Intuitively, $p_t^\prime(j) = \nicefrac{p_t(y=j)}{\sum_k p_t(y=k)}$ is
% re-normalized label distribution in target among previously seen classes and 
% $w(j)$'s are the 
% % re-normalized 
% importance ratios. 
% % For ease of notation, we refer $p_t^\prime(y)$ as the re-normalized label distribution 
% % among previously seen classes, i.e., 
% % $p_t^\prime(y = j) = {p_t(y=j)}/{\sum_k p_t(y=k)}$. 
% % 
% Hence, after obtaining label shift corrected source 
% distribution $p_s^\prime(x)$, 
% OSLS problem is reduced 
% to a \emph{single} instance of PU learning problem 
% where $p_s^\prime(x)$ can be considered as
% positive distribution and $p_t(x| y=k+1)$
% as negative distribution with mixture coefficients
% $1 - p_t(y=k+1)$ and $p_t(y=k+1)$ respectively. 
% Now we will discuss our methods to estimate
% the label shift among source classes (i.e. importance ratio's $w(y)$) and 
% tackle the PU learning instance obtained from OSLS.  
% % 


% While traditional methods for estimating label shift 
% breakdown in high dimensional settings~\citep{zhang2013domain, lipton2018detecting, azizzadenesheli2019regularized}, 
% recent methods exploit black-box classifiers to avoid curse of dimensionality~\citep{lipton2018detecting, azizzadenesheli2019regularized, garg2020unified, alexandari2019adapting}. 
% However, these recent techniques require overlapping label distributions, 
% and a direct application would require demarcation of samples from 
% $p^\prime_s(x)$ in target creating a cyclic dependency. 
% % 
% Instead, we build on recently proposed 
% Best Bin Estimation (BBE) 
% technique from \citet{garg2021PUlearning}. 
% Given positive and unlabeled data, 
% BBE estimates the fraction of positives in unlabeled 
% by leveraging a black-box classifier. 
% % 
% In particular, BBE identifies a threshold 
% on probability scores assigned by the classifier
% such that by estimating the ratio between
% the fractions of positive and unlabeled 
% points receiving scores above the threshold,
% we obtain proportion of positives in unlabeled.
% % 
% We tailor BBE to estimate
% the relative fraction of 
% previously seen classes in target 
% by exploiting a $k$-way source classifier $f_s$ trained 
% on labeled source data. 
% We describe the procedure in \appref{sec:OSLS_framework_app} (\algoref{alg:BBE}). 
% % 
% Note that, unlike in reduction of OSLS to $k$ PU problems, 
% we do not train $k$
% one-versus-other PU classifiers 
% and neither we use estimates of fraction 
% previously seen classes to directly estimate the novel class prevalence. \todosg{Check this and maybe cite experimental evidence?}


% After estimating the fraction 
% of source classes in target (i.e., $p_t^\prime(j) =\nicefrac{p_t(y=j)}{\sum_{k\in \out_s} p_t(y=k)}$ for all $j \in \out_s$), 
% we re-sample the source data according to $p_t^\prime(y)$
% to mimic samples from distribution $p_s^\prime(x)$. 
% Thus, obtaining a PU learning problem instance, 
% we next resort to PU learning techniques to 
% (i) estimate the fraction of novel class $p_t(y=k+1)$; 
% and (ii) learn a binary classifier $f_d(x)$ to discriminate 
% between label shift corrected source $p_s^\prime(x)$
% and novel class $p_t(x|y=k+1)$. 
% With traditional methods for PU learning
% involving domain discrimination, 
% over-parameterized models can
% memorize the positive instances 
% in unlabeled,
% assigning them confidently 
% to the negative class,
% which can severely hurt
% generalization on PN 
% data~\citep{kiryo2017positive, garg2021PUlearning}.
% Rather, we employ Conditional 
% Value Ignoring Risk (CVIR) loss
% proposed in \citet{garg2021PUlearning} 
% which was shown to outperform alternative 
% approaches. Given an estimate of 
% fraction of novel class $\wh p_t(y=k+1)$,
% CVIR objective discards the highest loss 
% $(1 - \wh p_t(y=k+1))$ fraction of examples
% on each training epoch, removing the 
% incentive to overfit to
% the examples from $p_s^\prime(x)$. 
% % 
% In particular, 
% we employ the iterative procedure
% that alternates between 
% estimating the prevalence 
% of novel class $\wh p_t(y=k+1)$ (with BBE) and 
% minimizing the CVIR loss with estimated 
% fraction of novel class. 
% % 
% We discuss this procedure in  
% detail in \appref{sec:OSLS_framework_app}.  

% Finally, to obtain a $(k+1)$-way classifier $f_t(x)$ on target 
% we combine discriminator $f_d$ and  source classifier $f_s$
% with importance-reweighted label shift correction. 
% In particular,
% for all $j \in \out_s$, $[f_t(x)]_j = (1 - f_d(x)) \frac{w(j) \cdot [f_s(x)]_j}{\sum_{k\in \out_s} w(k) \cdot [f_s(x)]_k} $
% and $[f_t(x)]_{k+1} = f_d(x)$. 
% Overall, our procedure can be summarized 
% as follows (\algoref{alg:PULSE}).
% % 
% First, we estimate the label shift among
% previously seen classes by leveraging 
% a source classifier $f_s$, 
% and then employ importance re-weighting of source 
% data to formulate a single PU learning problem 
% between source and target to estimate fraction 
% of novel class $\wh p_t(y=k+1)$ and 
% to learn a discriminator $f_d$ 
% for novel class. Combining discriminator 
% and label shift corrected source classifier
% we get $(k+1)$-way target domain classifier. 
% We theoretically analyse the PULSE framework in 
% \secref{sec:analysis}. \todosg{Finish this!}


% Our ideas for PULSE framework
% extend to separability 
% condition. 
% For separable 
% problems that do not 
% satisfy strong positivity, 
% % Note that,  
% equation
% \eqref{eq:label_shift_corr}
% continues to hold. 
% % 
% Hence, 
% we can aim to jointly 
% learn
% domain discriminator classifier
% and  label shift 
% among previously seen classes. 
% then employ recent
% label shift estimation techniques~\citep{lipton2018detecting,azizzadenesheli2019regularized,alexandari2019adapting} to estimate. 
% % 
% However, in our initial experiments,
% we observe that techniques proposed 
% under strong positivity were empirically 
% stable and outperform other baselines
% developed under separability.
% This is intuitive for many benchmark datasets 
% where for each class there exists a 
% subdomain that only belongs to that class. 
% % 
% We describe this in more detail in \appref{}. \todosg{Re check this?}
% % leave careful investigation for future work?


% % Moreover, 
% % We experimentally demonstrate the 
% % failure of this naive reduction  
% % in \secref{sec:exp}. 


==> Open set label shift (NeurIPS 2022)/sections/06_exp.tex <==



\textbf{Baselines {} {}} 
We compare PULSE with several popular methods from OSDA literature. While these methods are not specifically 
proposed for OSLS, they are introduced for the more general OSDA problem. In particular, we make comparions with DANCE~\citep{saito2020universal}, UAN~\citep{you2019universal}, CMU~\citep{fu2020learning}, STA~\citep{liu2019separate}, Backprop-ODA (or BODA)~\citep{saito2018open}. We use the open source implementation available at \url{https://github.com/thuml}.
% 
For alternative baselines, we experiment with source classifier directly deployed on the target data which may contain novel class and label shift among source classes (referred to as \emph{source-only}). We also train a domain discriminator classifier for source versus target (referred to as \emph{domain disc.}). This  is adaptation of PU learning baseline\citep{elkan2008learning} which assumes no label shift among source classes.
% is present in the target domain. 
Finally, per the reduction presented in \secref{sec:reduction}, we train $k$ PU classifiers (referred to as \emph{k-PU}).
We include detailed description of each method in \appref{subsec:baselines_app}. 


\textbf{Datasets {} {}} We conduct experiments with seven benchmark classification datasets across 
vision, natural language, biology and medicine. For each dataset, we simulate an OSLS problem as described in next paragraph.  
For vision, we use CIFAR10, CIFAR100 ~\citep{krizhevsky2009learning} and Entity30~\citep{santurkar2020breeds}. 
% Entity30 is a subset of ImageNet~\citep{russakovsky2015imagenet} with 30 super classes.   
% 
For language, we experiment with Newsgroups-20~(\url{http://qwone.com/~jason/20Newsgroups/})
dataset. 
% Our choices of datasets are motivated by the practical applications of OSLS. 
% 
% For example, as in a simulated setup of Newsgroups-20 data, in practice, novel news categories can appear over time but the distribution of articles given a news category might stay relatively unchanged. 
Additionally, inspired by applications of OSLS in biology and medicine, we experiment with Tabula Muris~\citep{tabula2020single} (Gene Ontology prediction), Dermnet (skin disease prediction~\url{https://dermnetnz.org/}), and BreakHis~\citep{spanhol2015dataset} (tumor cell classification). 
% 
% 
% 
% 
These datasets span language, image and table modalities. We provide interpretation of OSLS problem for each dataset along with other details in \appref{subsec:datasets_app}. 

\textbf{OSLS Setup {} {}} To simulate an OSLS problem, we experiment with different fraction of novel class prevalence, source label distribution, and target label distribution. We randomly choose classes that constitute the novel target class. 
% 
After randomly choosing source and novel classes, we first split the training data from each source class 
randomly into two partitions. This creates a random label distribution for shared classes among source and target. We then club novel classes to assign them a new class (i.e. $k+1$). %and club it with target data. 
Finally, we throw away labels for the target data to obtain an unsupervised DA problem. We repeat the same process on iid hold out data to obtain validation data with no target labels. 

\textbf{Training and Evaluation {} {} } We use Resnet18~\citep{he2016deep} for CIFAR10, CIFAR100, and Entity30. For newsgroups, we use a convolutional architecture. For Tabular Muris and MNIST, we use a fully connected MLP. For Dermnet and BreakHis, we use Resnet-50. For all methods, we use the same backbone for discriminator and source classifier. For kPU, we use a separate final layer for each class with the same backbone. We use default hyperparameters for all methods. 
%   
% 
For OSDA methods, we use default method specific hyperparameters introduced in their works. 
% 
Since OSDA methods do not estimate the prevalence of novel class explicitly,
we use the fraction of examples predicted in class $k+1$ as a surrogate. 
% 
We train models till the performance on validation source data (labeled) ceases to increase. Unlike OSDA methods, note that we do not use early stopping based on performance on held-out labeled target data.  
% 
To evaluate classification performance, we report target accuracy on all classes, seen classes and the novel class. For novel class prevalence estimation, we report absolute difference between the true and estimated marginal. 
% 
% 
We open-source our code and 
% at \url{https://github.com/Neurips2022Anon}. 
% since, we use fixed hyperparameters for all settings, 
by simply changing a single config file, new OSLS setups can be generated and experimented with. We provide precise details about hyperparameters, OSLS setup for each dataset and code in \appref{subsec:setup_app}.

 

% Next, we empirically evaluate performance of our proposed approach for both estimation and classification.
% the prevalence of novel class and .  

\begin{table}[t]
  \centering
  \small
%   \tabcolsep=0.12cm
  \setlength{\tabcolsep}{2pt}
  \renewcommand{\arraystretch}{1.2}
  \caption{\emph{Comparison of PULSE with other methods}. Across all datasets, PULSE outperforms alternatives for both target classification and novel class prevalence estimation. 
  Acc~(All) is target accuracy, Acc~(Seen) is target accuracy on examples from previously seen classes, and Acc~(Novel) is recall for novel examples. MPE~(Novel) is absolute error for novel prevalence estimation.  
%   
  Results  reported by averaging across 3 seeds.   
    Detailed results for each dataset with all methods in \appref{subsec:results_paper_app}.}\label{table:results}
  \vspace{5pt}
  \begin{tabular}{@{}*{11}{c}@{}}
  \toprule
   & & \multicolumn{4}{c}{\textbf{CIFAR-10}} & & \multicolumn{4}{c}{\textbf{CIFAR-100}}   \\
    \multirow{2}{*}{Method} & &   \multirow{2}{*}{  \parbox{1.cm}{\centering Acc (All)}} & \multirow{2}{*}{  \parbox{1.cm}{\centering Acc (Seen)}} & \multirow{2}{*}{  \parbox{1.cm}{\centering  Acc (Novel)}} & \multirow{2}{*}{  \parbox{1.cm}{\centering MPE (Novel)}} & &  \multirow{2}{*}{  \parbox{1.cm}{\centering Acc (All)}} & \multirow{2}{*}{  \parbox{1.cm}{\centering Acc (Seen)}} & \multirow{2}{*}{  \parbox{1.cm}{\centering Acc (Novel)}} & \multirow{2}{*}{  \parbox{1.cm}{\centering MPE (Novel)}} \\
    & & & & & & & & \\
  \midrule
  Source-Only && ${67.1}$ & $87.0$ & - & - && $46.6$ & $66.4$ & - & - \\
  \midrule 
  UAN~\citep{you2019universal}   && $15.4$ & $19.7$ & $25.2$ & $0.214$ && $18.1$ & $40.6$ & $14.8$ & $0.133$\\
  BODA~\citep{saito2018open} && $63.1$ & $66.2$ & $42.0$ & $0.162$ && $36.1$ & $17.7$ & $81.6$ & $0.41$\\ 
  DANCE~\citep{saito2020universal} && $70.4$ & $85.5$ & $14.5$ & $0.174$ && $47.3$ & $66.4$ & $1.2$ & $0.28$  \\
  STA~\citep{liu2019separate} && $57.9$ & $69.6$ & $14.9$ & $0.124$ && $42.6$ & $48.5$ & $34.8$ & $0.14$\\
  CMU~\citep{fu2020learning} && $62.1$ & $77.9$ & $41.2$ & $0.183$ && $35.4$ & $46.0$ & $15.5$ & $0.161$\\
  \midrule
  Domain Disc.~\citep{elkan2008learning} && $47.4$ & $87.0$ & $30.6$ & $0.331$ && $45.8$ & $66.5$ & $39.1$ & $\bf{0.046}$\\
  $k$-PU && $83.6$ & $79.4$ & $\bf{98.9}$ & $0.036$ && $36.3$ & $22.6$ & $\bf{99.1}$ & $0.298$  \\ 
  PULSE (Ours) && $\bf{86.1}$ & $\bf{91.8}$ & $88.4$ & $\bf{0.008}$ && $\bf{63.4}$ & $\bf{67.2}$ & $63.5$ & $0.078$ \\ 
  \bottomrule 
  \end{tabular}  
%   \vspace{-5pt}
%   \caption{ }\label{table:results_CIFAR}
\end{table}

\begin{table}[t]
  \centering
  \small
%   \tabcolsep=0.12cm
  \setlength{\tabcolsep}{1.5pt}
  \renewcommand{\arraystretch}{1.2}
%   \caption{Across all datasets PULSE significantly outperforms alternatives for both target classification and novel class prevalence estimation. Results
%     reported by averaging across 3 seeds. Detailed results for each dataset with all methods in \appref{subsec:results_paper_app}.}\label{table:results_bio}
%   \vspace{-5pt}
  \begin{tabular}{@{}*{16}{c}@{}}
  \toprule
   &   
   \multicolumn{2}{c}{\textbf{Entity30}} & 
   \multicolumn{2}{c}{\textbf{Newsgroups20}}  &  
   \multicolumn{2}{c}{\textbf{Tabula Muris}} &  
   \multicolumn{2}{c}{\textbf{BreakHis}} & 
   \multicolumn{2}{c}{\textbf{DermNet}}   \\
    \multirow{2}{*}{Method} 
     &    \multirow{2}{*}{  \parbox{1.0cm}{\centering  Acc (All)}}  &  \multirow{2}{*}{  \parbox{1.cm}{\centering MPE (Novel)}} 
      &   \multirow{2}{*}{  \parbox{1.0cm}{\centering  Acc (All)}}  &  \multirow{2}{*}{  \parbox{1.cm}{\centering MPE (Novel)}} 
    &    \multirow{2}{*}{  \parbox{1.0cm}{\centering  Acc (All)}}  &  \multirow{2}{*}{  \parbox{1.cm}{\centering MPE (Novel)}} 
    &  \multirow{2}{*}{  \parbox{1.0cm}{\centering  Acc (All)}}  & \multirow{2}{*}{  \parbox{1.cm}{\centering MPE (Novel)}}
    &  \multirow{2}{*}{  \parbox{1.0cm}{\centering  Acc (All)}} & \multirow{2}{*}{  \parbox{1.cm}{\centering MPE (Novel)}} \\
    & & & & & & & & & \\
  \midrule
  Source-Only & $32.0$ & - & $39.3$ & - & $33.8$ &  - & $70.0$ & - & $41.4$  & - \\
  \midrule 
  BODA~\citep{saito2018open} & $42.2$  & $0.189$ & $43.4$ & $0.16$ & $76.5$ & $0.079$ &  $71.5$ &  $0.077$ & $43.8$ & $0.207$\\
  \midrule
  Domain Disc. & $43.2$ & $0.135$ & $50.9$ & $0.176$& $73.0$ & $0.071$ & $56.5$& $0.091$ & $40.6$  & $0.083$\\
  $k$-PU & $50.7$ & $0.394$  & $52.1$ & $0.373$ & $85.9$ & $0.307$ & $75.6$ & $\bf{0.059}$ & $46.0$  & $0.313$ \\ 
  PULSE (Ours) & $\bf{58.0}$ & $\bf{0.054}$  & $\bf{62.2}$ & $\bf{0.061}$ & $\bf{87.8}$ & $\bf{0.058}$ & $\bf{79.1}$ & $\bf{0.054}$ & $\bf{48.9}$ & $\bf{0.043}$\\ 
  \bottomrule 
  \end{tabular}  
%   \vspace{-5pt}
\end{table}




\textbf{Results {} {}} Across different datasets, we observe that PULSE consistently outperforms other methods for the target classification and novel prevalence estimation (\tabref{table:results}). For detection of novel classes (Acc~(Novel) column), kPU achieves superior performance  
as compared to alternative approaches because of its bias to default to $(k+1)^\text{th}$ class. This is evident by the sharp decrease in performance on previously seen classes.  
% 
% 
% 
For each dataset, we plot evolution of performance with training in~\appref{subsec:results_paper_app}. We observe 
more stability in performance of PULSE as compared to other methods. 
% 
% in target accuracy and prevalence estimation with training. 


% \textbf{Failure of open set classification methods {} {}}


We observe that with
% out
% performing any
default hyperparameters, 
popular OSDA methods significantly 
under perform as compared to PULSE. 
We hypothesize that the primary reasons 
underlying the poor performance 
of OSDA methods are (i) the heuristics 
employed to detect novel classes; and 
(ii) loss functions incorporated to 
improve alignment between examples from 
common classes in source and target.
To detect novel classes, 
a standard heuristic employed in 
popular OSDA methods involves 
thresholding uncertainty 
estimates (e.g., prediction entropy, 
softmax confidence~\citep{you2019universal,fu2020learning,saito2020universal}) 
at a predefined 
threshold $\kappa$. However, 
a fixed $\kappa$, may not 
for different datasets and 
different fractions of 
the novel class. In \appref{subsec:OSDA_app}, 
we ablate by (i) removing loss function terms 
incorporated with an aim to improve source 
target alignment; and (ii) vary threshold
$\kappa$ and show improvements in performance 
of these methods. 
In contrast, our two-stage method 
PULSE, first estimates 
the fraction of novel class which 
then guides the classification 
of novel class versus previously seen classes
avoiding the need to guess $\kappa$. 

\textbf{Ablations {} {}}  
Different datasets, in our setup span different fraction of novel class prevalence ranging from $0.22$ (in CIFAR10) to $0.64$ (in Tabula Muris). For each dataset, we perform more ablations on the novel class proportion in \appref{subsec:novel_class_app}.
% 
% 
For kPU and PULSE, in the main paper, we include results with BBE and CVIR~\citep{garg2021PUlearning}. In \appref{subsec:different_PU_app}, we perform experiments with alternative PU learning approaches and highlight the superiority of BBE and CVIR over other methods. 
% 
Moreover, since we have access to unlabeled target data, we experiment with SimCLR~\citep{chen2020simple} pre-training on the mixture of unlabeled source and target dataset. We include setup details and results in \appref{subsec:contrastive_app}. While pre-trained backbone architecture improves performance for all methods, PULSE continues to dominate other methods.  



% \paragraph{Choices with other PU learning methods}



% \begin{table}[t]
%   \centering
%   \small
% %   \tabcolsep=0.12cm
%   \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{1.2}
%   \begin{tabular}{@{}*{11}{c}@{}}
%   \toprule
%   & &  \multicolumn{4}{c}{\textbf{Entity30}} & & \multicolumn{4}{c}{\textbf{Newsgroup20}}     \\
%   \multirow{2}{*}{Method} & &   \multirow{2}{*}{  \parbox{1.0cm}{\centering Acc (All)}} & \multirow{2}{*}{  \parbox{1.0cm}{\centering Acc (Seen)}} & \multirow{2}{*}{  \parbox{1.0cm}{\centering  Acc (Novel)}} & \multirow{2}{*}{  \parbox{1.0cm}{\centering MPE (Novel)}} & &  \multirow{2}{*}{  \parbox{1.0cm}{\centering  Acc (All)}} & \multirow{2}{*}{  \parbox{1.0cm}{\centering  Acc (Seen)}} & \multirow{2}{*}{  \parbox{1.0cm}{\centering  Acc (Novel)}} & \multirow{2}{*}{  \parbox{1.cm}{\centering MPE (Novel)}} \\ 
%     & & & & & & & & \\
%   \midrule
%   Source-Only && $32.0$  & $53.3$ & - & - && $39.3$ & $64.4$ & - & - \\
%   \midrule 
%   BODA~\citep{saito2018open} && $42.2$ & $33.4$ & $67.2$ & $0.189$ && $43.4$ & $34.7$ & $57.6$ & $0.16$\\
%   \midrule
%   Domain Disc. && $43.2$ & $53.3$ & $68.0$ & $0.135$ && $50.9$ & $64.4$ & $\bf{93.2}$ & $0.176$ \\
%   $k$-PU && $50.7$ & $22.3$ & $\bf{94.4}$ & $0.394$  && $52.1$ & $57.9$ & $42.2$ & $0.373$ \\
%   PULSE (Ours) && $\bf{58.0}$ & $\bf{53.6}$ & ${79.3}$ & $\bf{0.054}$  && $\bf{62.2}$ & $\bf{65.2}$ & ${82.2}$ & $\bf{0.061}$ \\ 
%   \bottomrule 
%   \end{tabular}  
%   \vspace{5pt}
%   \caption{ }\label{table:results_other}
% \end{table}


% \begin{table}[t]
%   \centering
%   \small
% %   \tabcolsep=0.12cm
%   \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{1.2}
%   \begin{tabular}{@{}*{14}{c}@{}}
%   \toprule
%   & &  \multicolumn{3}{c}{\textbf{Tabula Muris}} & & \multicolumn{3}{c}{\textbf{BreakHis}} & & \multicolumn{3}{c}{\textbf{DermNet}}     \\
%     \multirow{2}{*}{Method} 
%     & &   \multirow{2}{*}{  \parbox{1.0cm}{\centering  Acc (All)}} & \multirow{2}{*}{  \parbox{1.0cm}{\centering  Acc (Seen)}} &  \multirow{2}{*}{  \parbox{1.cm}{\centering MPE (Novel)}} 
%     & &  \multirow{2}{*}{  \parbox{1.0cm}{\centering  Acc (All)}} & \multirow{2}{*}{  \parbox{1.0cm}{\centering  Acc (Seen)}} & \multirow{2}{*}{  \parbox{1.cm}{\centering MPE (Novel)}}
%     & &  \multirow{2}{*}{  \parbox{1.0cm}{\centering  Acc (All)}} & \multirow{2}{*}{  \parbox{1.0cm}{\centering  Acc (Seen)}} & \multirow{2}{*}{  \parbox{1.cm}{\centering MPE (Novel)}} \\
%     & & & & & & & & & \\
%   \midrule
%   Source-Only && $33.8$ & $93.1$& - && $70.0$ & $95.8$ & - && $41.4$ & $53.6$ & - \\
%   \midrule 
%   BODA~\citep{saito2018open} && $76.5$ & $56.0$ & $0.079$ &&  $71.5$ & $81.9$ & $0.077$ && $43.8$ & $31.4$ & $0.207$\\
%   \midrule
%   Domain Disc. && $73.0$ & $93.1$ & $0.071$ && $56.5$ & $95.8$ & $0.091$ && $40.6$ & $53.6$ & $0.083$\\
%   $k$-PU && $85.9$ & $91.1$ & $0.307$ && $75.6$ & $71.7$ & $\bf{0.059}$ && $46.0$ & $26.1$ & $0.313$ \\ 
%   PULSE (Ours) && $\bf{87.8}$ & $\bf{93.6}$ & $\bf{0.058}$ && $\bf{79.1}$ & $\bf{96.1}$ & $\bf{0.054}$ && $\bf{48.9}$ & $\bf{53.8}$ & $\bf{0.043}$\\ 
%   \bottomrule 
%   \end{tabular}  
%   \vspace{5pt}
%   \caption{ }\label{table:results_bio}
% \end{table}

% \multicolumn{2}{c}{\textbf{Newsgroups-20}} & 

==> Open set label shift (NeurIPS 2022)/sections/07_analysis.tex <==
In this section, we analyse 
key steps of our PULSE procedure
for target label marginal estimation 
(Step 3, 5 \algoref{alg:PULSE})
and learning the domain discriminator 
classifier (Step 5, \algoref{alg:PULSE}). 
% 
Due to space constraints, we present informal results here 
and relegate formal statements and proofs to \appref{sec:OSLS_theory_app}.  

\paragraph{Theoretical analysis for target marginal estimation}
% 
Building on BBE results from \citet{garg2021PUlearning}, 
we present finite sample results
for target label marginal estimation. 
% 
When the data satisfies strong positivity, 
we observe that source classifiers often 
exhibit a threshold $c_y$ on softmax output of 
each class $y \in \out_s$ 
above which the \emph{top bin} (i.e., $[c_y, 1]$)
contains mostly examples from that class $y$. 
We give empirical evidence to this claim in \appref{sec:theorem1_proof}. 
% 
Then, we show that the existence 
of (nearly) pure top bin for each class in $f_s$
is sufficient for Step 3 in \algoref{alg:PULSE} 
to produce (nearly) consistent 
estimates:

\begin{theorem}[Informal] \label{thm:informal_BBE}
Assume that for each class $y\in \out_s$, there exists a threshold $c_y$
such that for the classifier $f_s$, if $[f_s(x)]_y > c_y$ for any $x$ then the true label 
for that sample $x$ is $y$. 
Then, we have $\norm{\wh p_t - p_t}{1} \le \calO\left(\sqrt{\nicefrac{k^3\log(4k/\delta)}{n}} + \sqrt{\nicefrac{k^2\log(4k/\delta)}{m}}\right)  \,$.
\end{theorem}

The proof technique simply builds on the proof of Theorem 1 in \citet{garg2021PUlearning}. 
By assuming that we recover close to ground truth label marginal 
for source classes, we can also extend the above 
analysis to Step 5 of \algoref{alg:PULSE}
to show convergence of estimate $\wh p_t(y=k+1)$ to true prevalence
$p_t(y = k+1)$. We discuss this further in \appref{sec:BBE_ext_app}.  

\paragraph{Theoretical analysis of CVIR in population} 
While the CVIR loss was proposed in \citet{garg2021PUlearning}, 
no analysis was provided
for convergence of the iterative 
gradient descent procedure.
In our work, we show that in population 
on a separable Gaussian dataset,
CVIR will recover the optimal classifier. 

% To keep the notation simple,
We consider a 
binary classification problem 
where we have access to 
positive distribution (i.e., $p_p$), 
unlabeled distribution 
(i.e., $p_u \defeq \alpha p_p + (1-\alpha) p_n$), 
and mixture coefficient $\alpha$. 
% 
Making a parallel connection to 
Step 5 of PULSE,  
positive distribution $p_p$ here refers
to the label shift corrected source distribution 
$p_s^\prime$ and $p_u$ refers to $p_t = p_t(y=k+1) p_t(x|y=k+1) + (1 - p_t(y=k+1)) p_s^\prime(x)$.
Our goal is to recover the classifier 
that discriminates $p_p$ versus $p_n$ (parallel $p_s^\prime$ versus $p_t(\cdot|y=k+1)$).
% 

First we introduce some notation. For a classifier $f$ and loss function $\ell$ (i.e., logistic loss), define $\vr_\alpha (f) = \inf \{ \tau \in \Real: \Prob_{x\sim p_u}( \ell(x, -1; f) \le \tau) \ge 1 - \alpha \}$. 
Intuitively, $\vr_\alpha(f)$ identifies a threshold $\tau$ to capture bottom $1-\alpha$ fraction of the loss $\ell(x, -1)$ 
for points $x$ sampled from $p_u$.  
Additionally, define CVIR loss as $\calL (f, w) = \alpha \Expt{p_p}{\ell(x,1; f)} + \Expt{p_u}{w(x)\ell(x,-1; f)}$ for classifier $f$ and some weights $w(x) \in\{0,1\}$. 
%
Formally, given a classifier $f_t$ at an iterate $t$, CVIR procedure proceeds as follows: 
\begin{align}
    w_t(x) &= \indict{\ell(x, -1; f_t) \le \vr_\alpha(f_t)} \,,\label{eq:step1_CVIR}\\ 
    f_{t+1} &= f_t - \eta \grad \calL_f (f_t, w_t) \,. \label{eq:step2_CVIR}
\end{align}
% 

\update{We assume that $x$ are drawn from two half multivariate 
Gaussian with mean zero and identity covariance, i.e., 
% \begin{align*}
    $x \sim p_p \Leftrightarrow x = \gamma_0 \theta_{\opt} + z | \, \theta_\opt^T z \ge 0,$ and  
    $x \sim p_n \Leftrightarrow x = -\gamma_0 \theta_{\opt} + z | \, \theta_\opt^T z < 0,  \text{ where } z \sim \calN(0, I_d)$.
% \end{align*}
Here $\gamma_0$ is the margin and $\theta_\opt \in \Real^d$ is the true separator. Here, we have access to distribution $p_p$, $p_u = \alpha p_p + (1 - \alpha) p_n$, and the true proportion $\alpha$.} 
% 
% Next, we show that  the CVIR procedure describe before 

% \vspace{-10pt}
\update{\begin{theorem}[Informal] \label{thm:informal_CVIR}
In the data setup detailed above, a linear classifier $f(x; \theta) = \sigma\left(\theta^Tx\right)$ trained with CVIR procedure as in \eqref{eq:step1_CVIR}-\eqref{eq:step2_CVIR} will converge to an optimal  positive versus negative classifier. 
% in direction, i.e., $\lim_{t \to \infty} \theta_t / \norm{\theta_t}{2} \to \theta_\opt$. 
% Minimizing the CVIR loss, i.e., \eqref{} in an iterative manner on population leads to the correct PvN classifier for separable datasets.  
\end{theorem}}

\update{The proof uses a key idea that for any classifier $\theta$ not separating positive and negative data perfectly, 
% in the direction of $\theta_\opt$,
the gradient in \eqref{eq:step2_CVIR} is non-zero. Hence, convergence of the CVIR procedure 
(implied by smoothness of CVIR loss) implies converge to an optimal classifier.} 
% 
For separable datasets in general, we can extend the above analysis with some modifications to the CVIR procedure. We discuss this in \appref{sec:CVIR_ext_app}.  

\paragraph{Empirical investigation in overparameterized models}
% 
As noted in our ablation experiments and in \citet{garg2021PUlearning}, 
domain discriminator trained with CVIR outperforms classifiers 
trained with other consistent objectives (nnPU~\citep{kiryo2017positive} and uPU~\citep{du2015convex}). 
% 
While the above analysis highlights consistency of CVIR procedure
in population, 
it doesn't capture the observed 
empirical efficacy of CVIR over 
alternative methods 
in overparameterized models. 
In the Gaussian setup described 
above, we train overparameterized 
linear models to compare CVIR with other methods.
% 
% 
We discuss precise experiments and results 
in \appref{sec:empirical_CVIR_app}, 
but highlight the key takeaway here. 
First, we observe that when a classifier 
is trained to distinguish positive and unlabeled
data, \emph{early learning}
happens~\citep{liu2020early,arora2019fine,garg2021RATT}, 
i.e., during the initial phase of learning 
classifier learns to classify 
positives in unlabeled correctly as positives.
Next, we show that post early learning  
rejection of large fraction of positives
from unlabeled training  
in equation \eqref{eq:step1_CVIR}
crucially helps CVIR. 

% \begin{figure*}[t!]
%   \centering 
%   % 
%   % \includegraphics[width=0.9\linewidth]{example-image-a}
%   \subfigure[Accuracy on validation positive versus negative data]{\includegraphics[width=0.4\linewidth]{figures/toy_acc.png}} \hfil
%   \subfigure[Fraction of correctly rejected examples with CVIR]{\includegraphics[width=0.4\linewidth]{figures/toy_rej.png}}
%   \caption{\textbf{Comparison of different methods in overparameterized toy setup.} CVIR (random) denotes CVIR with random initialization and CVIR (PvU) denotes warm start with a positive versus negative classifier. Vertical line denotes the epoch at which we switch from PvU to CVIR in CVIR (PvU) training. (a) We observe that CVIR (PvU) improves significantly even over the best early stopped PvU model. As training proceeds, we observe that accuracy of nnPU, uPU and PvU training drops whereas CVIR (random) and CVIR (PvU) maintains superior and stable performance. (b) We observe that warm start training helps CVIR over randomly initialized model to correctly identity positives among unlabeled for rejection. }
%   \label{fig:empirical_val}
%   % \vspace{-5pt}
% \end{figure*}

% Next,
% % the \emph{self-training} 
% % like objective of CVIR
% % \eqref{eq:step1_CVIR}, further improves the 
% % early learnt classifier. 
% we show that post early learning  
% rejection of large fraction of positives
% from unlabeled training  
% in equation \eqref{eq:step1_CVIR}
% crucially helps CVIR. 
% % performs empirically better than 
% % other consistent objectives nnPU~\citep{kiryo2017positive} and uPU~\citep{du2015convex}.



==> Open set label shift (NeurIPS 2022)/sections/08_conclusion.tex <==
In this work, we introduce OSLS a well-posed instantiation of OSDA
that subsumes label shift and PU learning
into a framework for learning adaptive classifiers.
We presented identifiability conditions 
for OSLS and proposed PULSE, 
a simple and effective approach 
to tackle the OSLS problem. 
Moreover, our extensive experiments 
demonstrate efficacy of PULSE 
over popular OSDA alternatives
when the OSLS assumptions are met. 
%
We would like to highlight the brittle nature 
of benchmark driven progress in OSDA 
% and with our work, 
and hope that our work can help to stimulate
more solid foundations and enable 
systematic progress in this area.
Finally, we hope that our open source code and benchmarks
will foster further progress on OSLS. 
% we hope to bring systematic progress
% in the field. 
% We should also note that 


\subsection{Limitations and Future Work}


\update{Here, we discuss limitations of the PULSE framework. First, to estimate the relative label shift among source classes in target, we leverage k-PU reductions with several modifications. While we reduce the issues due to overestimation bias by re-normalizing the label marginal among source classes in target, in future, we may hope to replace this heuristic step to directly estimate the joint target marginal.}

\update{Second, since our methods use CVIR and BBE sub-routines, failure of these methods can lead to failure of PULSE. For example, efficacy of BBE relies on the existence of an almost pure top bin in the classifier output space. While this property seems to be satisfied across different datasets spanning different modalities and applications, failure to identify an almost pure top bin can degrade the performance of BBE and hence, our PULSE framework.}  


In future work, we also hope to bridge the gap 
between the necessary and sufficient identifiability conditions. 
% 
While we empirically investigate reasons for CVIR's efficacy
in overparameterized models, 
we aim to extend our theory to overparameterized settings in future. 
In our work, we strictly operate under the OSLS settings, where we performed semi-synthetic experiments on vision, language and tabular datasets. In future, it will be interesting to experiment with our PULSE procedure in relaxed settings where $p(x|y)$ may shift in some natural-seeming ways from source to target. 

% 


% OK, I will fit this in 9 pages now, thanks :) 

%  In this work, we introduce OSLS, 
% a principled instantiation of OSDA problem. 
% Although OSLS setting 
% is relevant and simple,  
% it is largely unexplored. 
% We presented identifiability conditions 
% for OSLS and proposed PULSE, a simple yet effective 
% approach to tackle the OSLS problem. With extensive 
% experiments, we demonstrate efficacy of 
% PULSE over popular OSDA alternatives.
% %  
% We highlight
% the brittle nature of 
% benchmark driven progress in 
% OSDA and with our work, 
% we hope to bring systematic progress
% in the field. 
% % 
% In future work, we hope to bridge 
% the gap between the necessary and sufficient 
% identifiability conditions. 
% % 
% While we empirically investigate reasons for efficacy
% of CVIR 
% in overparameterized models, we aim 
% to extend our theoretical of CVIR procedure in population
% to overparameterized settings in future. 
% % 
% Finally, we hope that relevance of OSLS setup and 
% our open source code along with benchmark setup
% will foster progress 
% in this setting. 

 
